On how Cognitive Computing will plan your next Systematic Review

Systematic literature reviews (SLRs) are at the heart of evidence-based research, setting the foundation for future research and practice. However, producing good quality timely contributions is a challenging and highly cognitive endeavor, which has lately motivated the exploration of automation and support in the SLR process. In this paper we address an often overlooked phase in this process, that of planning literature reviews, and explore under the lenses of cognitive process augmentation how to overcome its most salient challenges. In doing so, we report on the insights from 24 SLR authors on planning practices, its challenges as well as feedback on support strategies inspired by recent advances in cognitive computing. We frame our findings under the cognitive augmentation framework, and report on a prototype implementation and evaluation focusing on further informing the technical feasibility.

==> Image/Backup/Implementation.tex <==
\indent{Collecting the Data}
Information related to systematic review is sourced is in unstructured, semi-structured, and structured formats and can be collected from multiple sources. The data comprises reviews' metadata ( e.g., title, authors, publication years), research questions as well as the SLR abstracts. Given that larger amounts of training data typically produce more accurate Word Embedding~\cite{mikolov2013distributed}, we propose to collect and leverage all these invaluable information sources into a database (namely MySQL). We implemented a REST API to save and retrieve raw and curated data.  
To process and transform data into semantically rich representations formats and stored in the data storage, before taking any step forward, we start with text pre-processing. The pre-processing segment comprises of two steps: (a) lemmatization: by converting each word within the corpus to its base form which we obtain Stanford CoreNLP toolkit ~\footnote{https://nlp.stanford.edu/software/tagger.html} to perform this process; and (b) normalization: by converting all the text into a more uniform sequence and removing the noise. We apply standard normalization techniques such as removing the special characters, punctuation, stop words, and numbers, followed by converting all characters to lowercase.\\  
% # Part 2 Word embedding and other services 
Following the data pre-processing step, the data curation is the next step that enables data extraction (e.g., extracting keywords and synonyms) and data enrichment (e.g., knowledge extraction, and recommendation). To achieve this, we leverage natural language processing (NLP) techniques~\cite{manning2014stanford,mikolov2013distributed} to process such textual data and finding hidden features. The inspiration behind our proposed approach is leveraging a similar approach to the word embedding's model~\cite{mikolov2013distributed} that represents words in a Vector Space Model (VSM). While general-purpose word embedding models often consider "word" as a vector, we have extended this idea to represent the SLR-related corpus (e.g., research questions and the SLR abstracts) in a vector space. After encoding the given corpus into vectors, they are used to calculate the similarity of the given corpus (such as calculating the similarity of a list of research questions and a list of abstracts). To create the VSMs, we employ an N-gram selector component to extract all the keywords (nouns and verbs) from sentences of the given context. We leverage Stanford Part-Of-Speech (POS) Tagger~\cite{manning2014stanford} to achieve this. We then create a list of n-grams out of these keywords and transform them into vector representations for each corpus.\\
To provide the facility to the end-users to utilize these embedding models as REST API, we leverage Flask technology~\footnote{https://flask-restful.readthedocs.io/en/latest/}. As an ongoing work, two of the APIs are publicly available. 

The first service is to compare and compute the similarity of the abstracts and the research questions, while the second provides the same service for comparing the abstracts and seeds abstract.


\indent{Aim.}
To ensure the uniqueness of a new proposed review, finding and assessing relevant systematic reviews is a necessary step in the planning phase. This task requires capturing the related properties of the publications, typically by matching keywords found in the title, abstract, or search by the topic. Cognitive knowledge is vital to translate the review scope into a viable set of query keywords. This task proves challenging and can take many iterations, involves trade-offs, and remain prone to error. In this experiment, we aim to evaluate the ability to use word embedding models from general language knowledge, to find systematic reviews that answer the research question without manually translating research questions into search queries. Our work leverages state-of-the-art algorithms widely used in NLP communities. Several such algorithms \textbf{Glove}~\cite{pennington2014glove}, \textbf{Universal}~\cite{cer2018universal}, \textbf{Word2Vec}~\cite{mikolov2013efficient},\textbf{Numberbatch}~\cite{speer2016conceptnet}, \textbf{WikiNewsFast}~\cite{bojanowski2017enriching}, and \textbf{GoogleNews}~\cite{church2017word2vec}. \\

==> Image/Backup/RelatedWork.tex <==

% Marcos - important 
% \subsection{Studies on challenges and barriers in the SLR process}
% The challenges in the SLR process have been studied from different perspectives and using the most varied set of methods.

% Carver et al.~\cite{carver2013identifying} conducted a study to identify the most challenging and time-consuming tasks in SLR process. Through an online survey they collected information related to the experience of 52 authors of SLRs in Software Engineering, focusing on seven main tasks. Their study also complemented this view with the experience of eight PhD students running SLRs in the context of a graduate course. The report 
% highlighted some challenges in the process and the importance of further collaboration on the planning and execution of the SLR to reduce the time, effort and potential errors. The experience from students also point to the need for more expert support. While this work provides valuable insights and serves as an inspiration for the current study, it differs in some meaningful ways. Unlike Carver et al.~\cite{carver2013identifying}, i) we systematically explore the phases and tasks associated to the SLR process adopting as a framework a widely followed reference process and set of guidelines \cite{Kitchenham2007}, ii) we adopt a broader perspective to inquire not only about the challenges but also their underlying reasons and the role played by technological support. We should also note that in the seven years since this survey, challenges and perspectives might have shifted, along with advancements in technology support. 

% Other researchers have looked for signs of issues in the SLR process by looking directly at published SLRs in Software Engineering.  
% %
% Imtiaz et al. \cite{imtiaz2013tertiary} performed a tertiary study to collect insights from SLRs that had included notes regarding their experience with the process. The ultimate goal was to record experiences that will benefit new researchers embarking in SLRs. The study collected perspectives from 116 studies to combine them in 11 themes. However, the resulting report focuses on the number of issues by theme, giving details on the derived challenges only for the definition of the "search strategy", which emerged as the most problematic one.
% Similarly, Palomino et al. \cite{palomino2018methodologies} looked at SLRs to characterise the most common difficulties in their elaboration, but by analysing the resulting quality of the papers. These two works provide an interesting approach to analysing the SLR process, but limited to assessing the end product. Inquiring about the reasons behind observed challenges, technology support, and mitigation strategies was  not the focus. 

% Another source of insights come from aggregating informed opinions by experts. 
% %
% Kitchenham and Brereton \cite{kitchenham2013systematic} synthesize lessons learned from 9 opinion papers reporting on problems in the SLR process. This is done in the context of their larger efforts in informing updates to SLR guidelines in Software Engineering. 
% Three main issues emerged related to digital libraries not providing adequate support, the effort in the process, and quality assessment issues. Given their targeted focus, the analysis did not take into account the reasons behind the challenges, perspectives from novice researchers, and tools and strategies to mitigate these issues. 
% %
% Garousi and Felderer~\cite{garousi2017experience} also rely on a similar approach but building on their own experience. They report on challenges and heuristics to address those challenges, as emerge from their experience in participating in 16 SLRs. Although insightful, their account is limited in scope, and focuses on   general challenges categories as they emerge from their experience, without the SLR process and tasks as the framework.

% Studies have also focused on the specific challenges faced by novice researchers.  Riaz et al.~\cite{riaz2010experiences} report on their experience running three SLRs as novice researchers and compare it to the experience of an expert. 
% %Through an experimental study, Riaz et al.~\cite{riaz2010experiences}reported the comparison result of experiences from three PhD students with carrying out SLRs to the experience of the senior researchers when undertaking an SLR. 
% They aimed to understand if the challenges faced by novices in terms of time taken to conduct the review is different from those faced by expert researchers. They reported that while some problems are faced by both novices and experts, many others are specific to novices, where the help of domain and SR experts can solve some of these issues. 
% %
% In the same vein, Ribeiro et al. \cite{ribeiro2018challenges}
% focus on challenges from the perspective of novices but
% by actually piloting an SLR protocol with different groups of students and observing differences in execution. Aside from the focus on novice researchers and the difference in methods (differences shared with the former study), the paper only focuses on the actual conduction of the SLR, as the review protocol, including all artefacts from the planning phase, were provided to the students. 

% Workshops have also been organized to collect perspectives from SLR authors.  Hassler et al. \cite{hassler2014outcomes} reports on the
% results from a workshop with 13 participants, including 11 senior and 2 novice researchers, all of them with previous SLR experience and active in the software engineering community. Their report addresses the barriers to completing an SLR, organised in barriers related to  the SLR process, to primary studies, to practitioners and tooling. Although definitely valuable, and addressing important issues, the discussions are centered around the the perspective of experts, limited in scope (e.g., missing collaboration aspects) and discussion on support tools. In a follow up \cite{hassler2016identification}, the authors report on identifying  SLR tool needs. However, it does not report on the experience and barriers in using and adopting actual SLR tools.

% The above has contributed to advancing our knowledge about the challenges and barriers in the SLR process, incorporating researchers' experience through different channels. In this work, however, we take a deeper look at examining the reasons behind those challenges, reflecting on the role of the experience in the process, as well as opportunities and barriers for technology-supported collaboration and automation.    

% Marcos  - important


%Despite many studies showing the common challenges of conducting SLR, none of these studies focused on the rationals behind these challenges. Yet, in this study, we aim at increasing our empirical knowledge on this field by a quantitative research. We gather and analyze the real challenges and reasons behind them. We also explore the solutions that the members of the research community employ to overcome these challenges. 

%Focusing on specific tasks associated to the SLR process.
%
%In a related work, Al-Zubidy et al.~\cite{al2019identification} investigated the challenges associated with the SLR search process. In their study, they conducted an SLR and surveyed SLR authors of the software engineering (SE) community. They compared the result of their SLR to the outcome of the survey to find the correlation between the problems identified by the literature to the real issues among the SLR authors.The authors also reported the desired tools requirements for the SLR search phase as a result of their survey. They showed that SLR search process in the SE domain still experiences a large number of barriers, and there is still the need for additional work towards automating this process.

% Impact on the SLR outcome
% coverage
% replicability
% timelesness


%Furthermore, previous research investigated on challenges of conducting SLR in diverse demographics of the research community. 

%Sandy Oliver et al.~\cite{oliver2015capacity} explored these challenges in the healthcare domain within low and middle-income countries (LMICs). They explored the current capacity and the activities that could improve SLR production in these countries. The result of their study showed that the limited capacity for conducting systematic reviews within LMICs presents a major challenge to improving their health systems. They also presented that effective capacity in these countries can be developed through funding at multiple levels simultaneously, supported by high-income countries with established facilities and expertise.
In this section, we compare and differentiate our work to previous research that focused on solutions to mitigate SLR challenges:\\
% \subsection{Collaboration and automation in the SLR process}
Extensive work has been done by the Software Engineering research community, and the research community in general, to alleviate SLR-related challenges. The efforts can be summarised in devising standard guidelines, supporting collaboration within and outside teams, and providing support tools and automation.
% what we know about collaboration
% tools supporting collaboration
%\cite{barn2014slrtool}
The literature includes remarkable examples of research collaboration enabled by technology. In Polymath~\cite{cranshaw2011polymath} mathematicians of different levels of seniority collaborate supported by mix of blog systems and wikis, producing scientific publications; in the Galaxy Zoo Quench project, citizen scientists were invited to research and write a paper on ``quenched" galaxies with the project scientists \cite{mitchell2018coordinating}; in Crowd Research \cite{vaish2017crowd} learning communities are leveraged to involve students across the globe in large scale research projects. While these are extreme examples of collaboration, they highlight opportunities and challenges that are also relevant when embarking in SLRs with larger teams. The role of collaboration in SLR has been acknowledged in previous works. The common view is that it is fundamental aspect needed along the entire SLR process \cite{al2017vision,hassler2016identification}. Hassler et al.~\cite{hassler2016identification} in their study of emerging needs for SLR support tools ranked collaboration among the top, listing collaboration among the SLR team, role management, dispute resolution and coordination as the desired features. Emerging from the challenges in the SLR process, collaboration has been hinted as possible solution for facilitating support for novice researchers \cite{riaz2010experiences}, putting SLR authors in contact with authors of primary studies \cite{riaz2010experiences,imtiaz2013tertiary} and enabling peer reviewing to reduce researcher bias \cite{garousi2017experience}. Reporting on actual experiences of collaboration and collaboration support tools in SLR is still an area requiring further studies.
The 
Most of the literature focus on aiding the study searching and citation screening by employing classification models. The common aim of these literature is to reduce the work-load or speed the SLR progress. One of the techniques that is used to reduce the workload of citation screening is visual text mining (VTM), which is largely championed by Felizardo et al.~\cite {felizardo2014visual}. They presented and evaluated the power of visualization techniques to aid SLR study identification in EBSE SLRs. They implemented a tool called "Revis" powered with VTM to help the citation screening. In another study, Fabbri et al.\cite{fabbri2016improvements} implemented a tool called "StArt" that employs VTM along with other text mining and information retrieval(IR) techniques to aid SLR tasks. They aimed to boost the reviewers' citation screening speed by reducing the number of studies that reviewers need to screen. "Rayyan" is another  platform that is built on top of a cloud-based, multi-tier service-oriented elastic architecture that predicts the studies relevant to aid citation screening ~\cite{ouzzani2016rayyan}. Similarly, Almeida et al.~\cite{Almeida2016} proposed  machine learning techniques to reduce the workloads of citation screening and applying inclusion/exclusion criteria tasks. Similarly, Marcos et al.\cite{marcos2018decision} adopted some machine learning algorithms and text mining techniques to extract relevant terms from the studies abstracts to support the process of building search queries. Lang et al.~\cite{langlois2018} also proposed a machine learning classification model to determine the empirical and non-empirical studies. In another study, Ghafari et al.~\cite{ghafari2012federated} presented a tool and used a data retrieval technique to help with query building and search multiple libraries at once and retrieve the results from different databases in a useful format. 
"Abstrackr" is also an online tool to support citation screening in SLR with employing machine learning methods(such as active learning) to interactively classify studies~\cite{Wallace2017}. The other group of research focused on automation the date extraction. Guo et al.~\cite{guo2016extracting} proposed a method for extracting synthesized claim sentences from the systematic reviews and the included primary studies. They proposed a method to use machine learning model to predict if the result of a newly published study will change the claim result of a published SLR. In another study, Bui et al.~\cite{bui2016extractive} proposed a text summarization method to enhance productivity and reduce errors in the traditional data extraction process for Medical SLRs. This model utilizes machine learning techniques to automatically generate summaries of the article's full-text. One another tool that is implemented to help with data extraction task is~"SparkText", a data mining framework to extract information from biomedical studies~\cite{ye2016sparktext}. 
Despite the existing enthusiasm for developing automation tools to aid this process, we know little about the pace of delivering the SLR tools into the consumer-level and adoption rate of this tools and automation techniques in the real SLR scenarios. We also keen to know if tools can adopted across disciplines with minimum twist.
With the advancements in automation techniques (e.g., data mining and machine learning) the research community spent a considerable endeavor in employing these techniques and developing tools for aiding the SLR process. Several projects focus on automating and streamlining specific SLR tasks. Some tasks received more automation aids while others are still largely manual.  The state of the art of information systems designed to support or automate SLR tasks implies the importance of this research topic. 
The above studies tell us that there is a place and demand for support tools in the SLR process. However, there is a need for a better understanding of the role of technology, especially in regards to new large-scale collaboration and automation opportunities, in current practice. 
In this 

% what we know about crowdsourcing
% tools supporting crowdsourcing
% Crowdsourcing has also been explored as an approach to scale efforts related to the SLR process, but with a focus on simpler repetitive tasks. It has been explored to support the screening of abstracts by relying on a crowd of non-experts~\cite{brown2014using,mortensen2017exploration}, in some cases optimising the assignment of papers with machine learning support \cite{krivosheev2018combining,nguyen2015combining}, or to support other tasks such as information extraction from papers~\cite{sun2016crowdsourcing}. 
% These experiments and other ongoing efforts report on promising results in terms of performance, contributing with tasks designs and guidelines for supporting specific aspects of the SLR process. These lessons learned can be leveraged nowadays by designing tasks on crowdsourcing platforms such as Amazon Mechanical Turk\footnote{\url{https://www.mturk.com/}}, Yandex Toloka\footnote{\url{https://toloka.yandex.com/}}, or specific support tools for crowdsourced SLR tasks (e.g., \cite{ramirez2018crowdrev}). Despite the potential of crowdsourcing for SLRs, we know little about if and to what extent it is adopted by researchers in their SLR processes and barriers preventing them from using it. 

% acceptance in research
% \cite{law2017crowdsourcing}

% \textbf{xxxxxxxxxx This needs to be properly extended}
% There are several active research groups across different research disciplines such as medicine ~\cite{Wallace2017,marshall2018machine,cohen2015automated} and software Engineering~\cite{felizardo2014visual}.


% Also knowing that some of these tools are designed for a specific research domain if the lessons learned through pioneers can be adopted in other domains. 

% This may be prevented by several factors such as missing the collaboration between the tool developers and the SLR authors. The tool developers require to attain the pain-points that authors face when conducting SLR, rather than implementing tools that are complex to use and rarely used in real SLR scenarios.

%and the second group who are exploring the advantage of employing the crowds to help within this





% Future research Research is needed on the design and evaluation of specialized question-answering systems that accept the nuances of systematic review questions, use search filters and strategies to search multiple databases to find the relevant systematic review or systematic review protocol.


==> Image/Backup/Technical.tex <==

% In this section, we present the prototype that we implemented and to evaluate the proposed framework.
% In the following, we identify some of the relevant cognitive support areas:
% % 1.what did we prototype and why ?
% We started with the The system allows users togo from their (partial) RQs directly to similar SLRs and seed papers

% We designed our framework (SLR-PRO) based on the cognitive process vision that augments the current SLR process with the vibrant and already mature advances in data curation and machine learning. 


Fig.~\ref{fig:Pipeline} presents the pipeline of the implementation. Next, we elaborate on the prototype implementation steps:\\
\begin{figure}
\centering
    \includegraphics[width=\textwidth]{Image/Pipeline.pdf}
\caption{Conceptual Architecture for Cognitive Augmentation in SLR Process} \label{fig:Pipeline}
\end{figure}
% # Part one Data , Data management , Pre-processing
\indent\textbf{Data Pre-Processing and Cleaning}
% \indent\textbf{Service Layer:} 


Information related to systematic review is sourced is in unstructured, semi-structured, and structured formats and can be collected from multiple sources.
Such information typically come in the form of reviews (

The data comprises reviews' metadata ( e.g., title, authors, publication years), research questions as well as the SLR abstracts. To manage the large amount of the invaluable data from an ever-increasing number of published SLRs, we  

we leverage the concept of Data Lake as a service as defined by Beheshti et al.~\cite{beheshti2017coredb}.

Data Lake serves as a high-capacity repository for any structured or unstructured data. The data lake service manages multiple database technologies to store and query data. By leveraging the SLR-PRO data curation component that we discuss next, in addition to raw data, curated data items are also stored in the data lake( e.g., extracting features such as keywords). 
To process and transform data into semantically rich representations formats and stored in the data storage, before taking any step forward, we start with text pre-processing. The pre-processing segment comprises of two steps: (a) lemmatization: by converting each word within the corpus to its base form which we obtain Stanford CoreNLP toolkit ~\footnote{https://nlp.stanford.edu/software/tagger.html} to perform this process; and (b) normalization: by converting all the text into a more uniform sequence and removing the noise. We apply standard normalization techniques such as removing the special characters, punctuation, stop words, and numbers, followed by converting all characters to lowercase.\\  % # Part 2 Word embedding and other services 
Following the data pre-processing step, the data curation is the next step that enables data extraction (e.g., extracting keywords and synonyms) and data enrichment (e.g., knowledge extraction, and recommendation). To achieve this, we leverage natural language processing (NLP) techniques~\cite{manning2014stanford,mikolov2013distributed} to process such textual data and finding hidden features. The inspiration behind our proposed approach is leveraging a similar approach to the word embedding's model~\cite{mikolov2013distributed} that represents words in a Vector Space Model (VSM). While general-purpose word embedding models often consider "word" as a vector, we have extended this idea to represent the SLR-related corpus (e.g., research questions and the SLR abstracts) in a vector space. After encoding the given corpus into vectors, they are used to calculate the similarity of the given corpus (such as calculating the similarity of a list of research questions and a list of abstracts). To create the VSMs, we employ an N-gram selector component to extract all the keywords (nouns and verbs) from sentences of the given context. We leverage Stanford Part-Of-Speech (POS) Tagger~\cite{manning2014stanford} to achieve this. We then create a list of n-grams out of these keywords and transform them into vector representations for each corpus.\\
% \indent\textbf{Application Layer:} 
% This middle layer contains the functional logic that drives the framework's core capabilities. This layer hosts embedding models.

It facilitates the exploration of several embedding models for the end-users' intended scenarios. To provide the facility to the end-users to utilize these embedding models as REST API, we leverage Flask technology~\footnote{https://flask-restful.readthedocs.io/en/latest/}. As an ongoing work, two of the APIs are publicly available. The first service is to compare and compute the similarity of the abstracts and the research questions, while the second provides the same service for comparing the abstracts and seeds abstract. We leverage publicly available embedding models to provide these services:
\textbf{Glove}~\cite{pennington2014glove}, \textbf{Universal}~\cite{cer2018universal}, \textbf{Word2Vec}~\cite{mikolov2013efficient},\textbf{Numberbatch}~\cite{speer2016conceptnet}, \textbf{WikiNewsFast}~\cite{bojanowski2017enriching}, and \textbf{GoogleNews}~\cite{church2017word2vec}. \\
% \begin{figure}
% \centering
% \includegraphics[width=0.9\textwidth]{Image/UI.JPG}
% \caption{SLR-PRO User Interface} \label{fig:UI}
% \end{figure}
\indent\textbf{Delivery Layer:}
Finally, the delivery layer is the front end layer in this 3-layer architecture and is the point of user interaction with the framework. This layer consists of different channels of accessing the provided services. At this stage of implementation, to invoke appropriate APIs, based on the intents detected by the chosen service; we implemented a landing page by leveraging Streamlit~\footnote{https://www.streamlit.io/} technology. The result of calling the APIs is then presented in a visual or tabular model to communicate information clearly and efficiently. Our next step of implementation is providing digital assistant to the end-user and supporting natural language interactions resembling by providing guidance, and recommendation, and contextualization SLR related information.\\ 
As stated before there are several use cases for this framework. Its flexibility provides the ground for being adopted in different scenarios. Next, we present the initial experiment we ran for one of these scenarios.
% question answering systems system , in which the answer to a research question is an SLR. 
\subsection{Experiment} % \subsection{Demonstration Scenario}
\noindent\textbf{Aim.} To ensure the singularity of a new review, finding and assessing relevant systematic reviews is a necessary step when planning a new review. This task requires capturing the related properties of the publications, typically by matching keywords found in the title, abstract, or search by the topic. Cognitive intelligence is vital to translate the review scope into a viable set of query keywords. This task proves challenging. This process can take many iterations, involve trade-offs, and be prone to error. In this experiment we aim to evaluate the ability of our approach of using word similarity algorithms word embedding models(by using word embeddings from general language knowledge) to find systematic reviews that answer the research question without manually translating research questions into search queries. We also aim to see the impact of using different word embedding models (that are trained on different corpora) on the performance of our framework.\\ 
% Automated support for this could be word similarity algorithms (by using word embeddings, either from general language knowledge or by specializing word vectors for a field of science). The word similarity models can then be leveraged for finding similar articles. The models can also be enhanced by maintaining by the domain expert feedback.
% This experiment aims to evaluate the ability of our approach to find systematic reviews that answer the research question without manually translating research questions into search queries. We also aim to see the impact of using different word embedding models (that are trained on different corpora) on the performance of our framework.\\ 
\noindent\textbf{Dataset.}

In our previous attempt to conduct a systematic review we searched for the relevant systematic reviews in digital libraries. As a result, we collected 250 published systematic reviews. Two researchers screened the reviews that resulted in finding only ten relevant reviews and 240 irrelevant. We used this dataset for this preliminary experiment~\footnote{All materials related to the experiment can be found at \textit{~\href{https://github.com/maisieb01/Cognitive_SLR.git}{DataSet}}}.\\
\noindent\textbf{Procedure.} One of the most popular methods for evaluating the quality of word embedding models is to assess how well the similarity scores of the word vectors correlate with human judgment~\cite{shi2017jointly}. Armed with the human-annotated dateset, explained before, we evaluate our approach by comparing the result of the similarity score of different embedding models with the result of the human. First, we call the SLR-PRO endpoint to calculate the similarity of research questions that we have defined for our SLR to a list of SLRs abstracts from the dataset. Second, we used the SLR-PRO API endpoint to calculate the similarity of the seed abstract to a list of SLRs abstracts from the dataset. For the seed abstract, we use our initial abstract from our systematic review. The similarity between documents is calculated as the distances between the vectors representing them. As suggested by ~\cite{lopes2007visual}, cosine similarity is more suitable for SLRs, therefore we follow the same approach. We use the common formulation \begin{equation}d(xi, xj)= 1 \text{-} \cos(xi, xj)\end{equation}, where xi and xj are the vectors representing the $i$th and $j$th documents(abstracts), respectively. Cosine similarity considers the vector space model (VSM) to measure the similarity between two documents. It is measured by the cosine of the angle between two vectors and defines whether two vectors are pointing in approximately the same direction~\cite{sidorov2014soft}.\\
\noindent\textbf{Metrics.} To evaluate the accuracy of our proposed approach, we used Spearman’s rank correlation. The Spearman’s rank correlation between our approach for similarity score and users annotations to evaluate how well the similarity of the given pairs (described above) agrees with human judgments~\cite{huang2012improving}. The higher the number, the stronger the correlations.\\
% Kappa compares an observed accuracy with an expected accuracy (random chance) in a confusion matrix. As it considers random chance, it is less misleading than using accuracy as a metric. Typical interpretation of such coefficient in relation to the agreement levels are~\begin{math} Poor(k  < 0.20), Fair (0.20 \le k < 0.40), Moderate (0.40 \le k < 0.60), Good (0.60 \le k < 0.80), Excellent (0.80 \le k \le 1.00)\end{math}.\\
\noindent\textbf{Preliminary Results.}
By computing the Spearman score obtained (rs = 0.67) indicates that our approach similarity score and the human ratings/score strongly correlated and well agreed with human judgement~\cite{huang2012improving}. To see the impact of using different word embedding models on the performance of finding the most relevant SLRs. The Universal model outperformed the other models when used by 
We evaluated the performance of our in terms of Precision and Recall - while using different word embedding models.

% Table.~\ref{table:Result} summarizes the results of our experiment. 
% \begin{table}
% \caption{Summary of Results.}\label{table:Result}
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% Model &  Precision & Recall\\
% \hline
% Glove &  1 & 14 point \\
% Universal &  2 & 12 point \\
% Word2Vec & 3 & 10 point \\
% Numberbatch & 4 & 10 point \\
% WikiNewsFast & 5 & 10 point \\
% GoogleNews& 6 & 10 point\\
% \hline
% \end{tabular}
% \end{table}


Beyond the positive results obtained in this work and possible application scenarios of our approach, we believe that there is still enough space for improvement. For future work, we intend to conduct other experiments using larger sample sizes of the dataset. We also aim to implement a virtual assistant (a.k.a chatbot) to interact with the users by using natural language queries. By leveraging our approach, stored SLR related information that is encoded into vectors where each vector is a representation of an SLR element (e.g. research questions, abstracts, authors name). Armed with such forms of data representation the chatbot can process users’ NL queries. The NL queries could be a research question and the response would be relevant SLRs.
% This step evaluates how well our approach agree with human judgements. For our preliminary investigation, we take a sample of 200-word pairs annotated by users on a Likert Scale, as mentioned in the previous step. Following SCWS dataset evaluation [17], we also compute the Spearman’s rank correlation between our word embedding similarity score and users annotations. The
% higher the number, the stronger the correlations. The score obtained (rs = 0.62) indicates that our WE similarity score and the human ratings/score strongly correlated and well agreed with human judgement [17].

% Word embedding originates from the distributional hypothesis~\cite{mikolov2013distributed}, which states that the words occurring in similar contexts tend to have similar meanings. Our work leverages state-of-the-art algorithms broadly used in NLP communities. Various such algorithms are available as libraries for popular programming languages such as Universal ~\cite{cer2018universal} and Word2Vec~\cite{mikolov2013efficient}. We adopt word2vec~\cite{mikolov2013efficient}, which comes in two variants, namely, Continuous Bag of-Words (CBOW) and Skip-Gram. From these two models, we leverage the Skip-gram model~\cite{manning1999foundations}. The Skip-gram model tries to predict the source context words (surrounding words) given a target word within a sliding window and map the words to a vector space. As an essential step that transforms raw text into a format suitable for further processing, we applied the standard pre-process techniques: tokenization, stop words/frequent words removal, and lemmatization for the given corpora.

% We use Stanford CoreNLP~\cite{manning2014stanford}

% This powerful feature is leveraged in the literature to develop robust semantic similarity techniques in various domains~\cite{de2016representation}

% (by using word embeddings, either from general language knowledge or by specializing word vectors for a field of science) and by using machine-learning classifiers to label reviews.

% Managing the endless amount of data from an ever-increasing number of published systematic reviews is a challenge for most of the researchers. SLR datasets are usually managed independently by research groups. They are often curated manually and consist of valuable information that can be used in future researchers. 

% \subsection{Enabler Layer}
% \subsection{Interface Layer}
% \section{Experiment}




==> Image/Backup/backup__Ref.tex <==
% 
@article{al2019identification,
  title={Identification and prioritization of SLR search tool requirements: an SLR and a survey},
  author={Al-Zubidy, Ahmed and Carver, Jeffrey C},
  journal={Empirical Software Engineering},
  volume={24},
  number={1},
  pages={139--169},
  year={2019},
  publisher={Springer}
}


@inproceedings{Peters:2018,
  author={Peters, Matthew E. and  Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  title={Deep contextualized word representations},
  booktitle={Proc. of NAACL},
  year={2018}
}



@inproceedings{le2014distributed,
  title={Distributed representations of sentences and documents},
  author={Le, Quoc and Mikolov, Tomas},
  booktitle={International conference on machine learning},
  pages={1188--1196},
  year={2014}
}




@article{cer2018universal,
  title={Universal sentence encoder},
  author={Cer, Daniel and Yang, Yinfei and Kong, Sheng-yi and Hua, Nan and Limtiaco, Nicole and John, Rhomni St and Constant, Noah and Guajardo-Cespedes, Mario and Yuan, Steve and Tar, Chris and others},
  journal={arXiv preprint arXiv:1803.11175},
  year={2018}
}







@article{hall2011systematic,
  title={A systematic literature review on fault prediction performance in software engineering},
  author={Hall, Tracy and Beecham, Sarah and Bowes, David and Gray, David and Counsell, Steve},
  journal={IEEE Transactions on Software Engineering},
  volume={38},
  number={6},
  pages={1276--1304},
  year={2011},
  publisher={IEEE}
}

@article{kitchenham2010systematic,
  title={Systematic literature reviews in software engineering--a tertiary study},
  author={Kitchenham, Barbara and Pretorius, Rialette and Budgen, David and Brereton, O Pearl and Turner, Mark and Niazi, Mahmood and Linkman, Stephen},
  journal={Information and software technology},
  volume={52},
  number={8},
  pages={792--805},
  year={2010},
  publisher={Elsevier}
}
@article{radjenovic2013software,
  title={Software fault prediction metrics: A systematic literature review},
  author={Radjenovi{\'c}, Danijel and Heri{\v{c}}ko, Marjan and Torkar, Richard and {\v{Z}}ivkovi{\v{c}}, Ale{\v{s}}},
  journal={Information and software technology},
  volume={55},
  number={8},
  pages={1397--1418},
  year={2013},
  publisher={Elsevier}
}

@article{wahono2015systematic,
  title={A systematic literature review of software defect prediction},
  author={Wahono, Romi Satria},
  journal={Journal of Software Engineering},
  volume={1},
  number={1},
  pages={1--16},
  year={2015}
}


@book{manning1999foundations,
  title={Foundations of statistical natural language processing},
  author={Manning, Christopher and Schutze, Hinrich},
  year={1999},
  publisher={MIT press}
}

@article{powers2011evaluation,
  title={Evaluation: from precision, recall and F-measure to ROC, informedness, markedness and correlation},
  author={Powers, David Martin},
  year={2011},
  publisher={Bioinfo Publications}
}






@article{sidorov2014soft,
  title={Soft similarity and soft cosine measure: Similarity of features in vector space model},
  author={Sidorov, Grigori and Gelbukh, Alexander and G{\'o}mez-Adorno, Helena and Pinto, David},
  journal={Computaci{\'o}n y Sistemas},
  volume={18},
  number={3},
  pages={491--504},
  year={2014},
  publisher={Centro de Investigaci{\'o}n en Computaci{\'o}n, IPN}
}



%added by maisie for short paper 

@article{Adeva2014,
author = {Garc\'{\i}a Adeva, J. J. and Pikatza Atxa, J. M. and Ubeda Carrillo, M. and Ansuategi Zengotitabengoa, E.},
title = {Automatic Text Classification to Support Systematic Reviews in Medicine},
year = {2014},
publisher = {Pergamon Press, Inc.},
doi = {10.1016/j.eswa.2013.08.047},
journal = {Expert Syst. Appl.},
pages = {1498–1508},
}

@article{Almeida2016,
author={H. {Almeida} and M. {Meurs} and L. {Kosseim} and A. {Tsang}},
journal={IEEE Transactions on NanoBioscience},
title={Data Sampling and Supervised Learning for HIV Literature Screening},
year={2016},
volume={15},
number={4},
pages={354-361},
doi={10.1109/TNB.2016.2565481},
ISSN={1558-2639},
}

@inproceedings{marshall2013tools,
  title={Tools to support systematic literature reviews in software engineering: A mapping study},
  author={Marshall, Christopher and Brereton, Pearl},
  booktitle={2013 ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={296--299},
  year={2013},
  organization={IEEE}
}

@article{Wallace2017,
  title={Identifying reports of randomized controlled trials (RCTs) via a hybrid machine learning and crowdsourcing approach},
  author={Wallace, Byron C and Noel-Storr, Anna and Marshall, Iain J and Cohen, Aaron M and Smalheiser, Neil R and Thomas, James},
  journal={Journal of the American Medical Informatics Association},
  volume={24},
  number={6},
  pages={1165--1168},
  year={2017},
  publisher={Oxford University Press}
}
@article{marshall2018machine,
  title={Machine learning for identifying randomized controlled trials: an evaluation and practitioner's guide},
  author={Marshall, Iain J and Noel-Storr, Anna and Kuiper, Jo{\"e}l and Thomas, James and Wallace, Byron C},
  journal={Research synthesis methods},
  volume={9},
  number={4},
  pages={602--614},
  year={2018},
  publisher={Wiley Online Library}
}
@inproceedings{felizardo2014visual,
  title={A visual analysis approach to update systematic reviews},
  author={Felizardo, Katia Romero and Nakagawa, Elisa Yumi and MacDonell, Stephen G and Maldonado, Jos{\'e} Carlos},
  booktitle={Proceedings of the 18th International Conference on Evaluation and Assessment in Software Engineering},
  pages={1--10},
  year={2014}
}
@inproceedings{fabbri2016improvements,
  title={Improvements in the StArt tool to better support the systematic review process},
  author={Fabbri, Sandra and Silva, Cleiton and Hernandes, Elis and Octaviano, F{\'a}bio and Di Thommazo, Andr{\'e} and Belgamo, Anderson},
  booktitle={Proceedings of the 20th International Conference on Evaluation and Assessment in Software Engineering},
  pages={1--5},
  year={2016}
}

@inproceedings{marcos2018decision,
  title={Decision support tools for SLR search string construction},
  author={Marcos-Pablos, Samuel and Garc{\'\i}a-Pe{\~n}alvo, Francisco Jos{\'e}},
  booktitle={Proceedings of the Sixth International Conference on Technological Ecosystems for Enhancing Multiculturality},
  pages={660--667},
  year={2018}
}

@inproceedings{guo2016extracting,
  title={Extracting Knowledge Claims for Automatic Evidence Synthesis Using Semantic Technology},
  author={Guo, Jinlong},
  booktitle={European Knowledge Acquisition Workshop},
  pages={238--244},
  year={2016},
  organization={Springer}
}


@article{bui2016extractive,
  title={Extractive text summarization system to aid data extraction from full text in systematic review development},
  author={Bui, Duy Duc An and Del Fiol, Guilherme and Hurdle, John F and Jonnalagadda, Siddhartha},
  journal={Journal of biomedical informatics},
  volume={64},
  pages={265--272},
  year={2016},
  publisher={Elsevier}
}

@article{cohen2015automated,
  title={Automated confidence ranked classification of randomized controlled trial articles: an aid to evidence-based medicine},
  author={Cohen, Aaron M and Smalheiser, Neil R and McDonagh, Marian S and Yu, Clement and Adams, Clive E and Davis, John M and Yu, Philip S},
  journal={Journal of the American Medical Informatics Association},
  volume={22},
  number={3},
  pages={707--717},
  year={2015},
  publisher={Oxford University Press}
}

@article{brown2014using,
  title={Using crowdsourcing to evaluate published scientific literature: methods and example},
  author={Brown, Andrew W and Allison, David B},
  journal={PloS one},
  volume={9},
  number={7},
  year={2014},
  publisher={Public Library of Science}
}

@article{kontonatsios2017,
  title={A semi-supervised approach using label propagation to support citation screening},
  author={Kontonatsios, Georgios and Brockmeier, Austin J and Przyby{\l}a, Piotr and McNaught, John and Mu, Tingting and Goulermas, John Y and Ananiadou, Sophia},
  journal={Journal of biomedical informatics},
  volume={72},
  pages={67--76},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{krivosheev2018,
  title={Crowd-based multi-predicate screening of papers in literature reviews},
  author={Krivosheev, Evgeny and Casati, Fabio and Benatallah, Boualem},
  booktitle={Proceedings of the 2018 World Wide Web Conference},
  pages={55--64},
  year={2018}
}
@article{langlois2018,
  title={Discriminating between empirical studies and non-empirical works using automated text classification},
  author={Langlois, Alexis and Nie, Jian-Yun and Thomas, James and Hong, Quan Nha and Pluye, Pierre},
  journal={Research synthesis methods},
  volume={9},
  number={4},
  pages={587--601},
  year={2018},
  publisher={Wiley Online Library}
}
@article{zhang2005domain,
  title={Domain Knowledge, Search Behaviour, and Search Effectiveness of Engineering and Science Students: An Exploratory Study.},
  author={Zhang, Xiangmin and Anghelescu, Hermina GB and Yuan, Xiaojun},
  journal={Information Research: An International Electronic Journal},
  volume={10},
  number={2},
  pages={n2},
  year={2005},
  publisher={ERIC}
}


@article{ye2016sparktext,
  title={Sparktext: Biomedical text mining on big data framework},
  author={Ye, Zhan and Tafti, Ahmad P and He, Karen Y and Wang, Kai and He, Max M},
  journal={PloS one},
  volume={11},
  number={9},
  year={2016},
  publisher={Public Library of Science}
}




@article{van2013overview,
  title={Overview of data-synthesis in systematic reviews of studies on outcome prediction models},
  author={van den Berg, Tobias and Heymans, Martijn W and Leone, Stephanie S and Vergouw, David and Hayden, Jill A and Verhagen, Arianne P and de Vet, Henrica CW},
  journal={BMC Medical research methodology},
  volume={13},
  number={1},
  pages={42},
  year={2013},
  publisher={Springer}
}

@article{lanera2018extending,
  title={Extending PubMed searches to ClinicalTrials. gov through a machine learning approach for systematic reviews},
  author={Lanera, Corrado and Minto, Clara and Sharma, Abhinav and Gregori, Dario and Berchialla, Paola and Baldi, Ileana},
  journal={Journal of clinical epidemiology},
  volume={103},
  pages={22--30},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{marcos2018decision,
  title={Decision support tools for SLR search string construction},
  author={Marcos-Pablos, Samuel and Garc{\'\i}a-Pe{\~n}alvo, Francisco Jos{\'e}},
  booktitle={Proceedings of the Sixth International Conference on Technological Ecosystems for Enhancing Multiculturality},
  pages={660--667},
  year={2018}
}
@inproceedings{goswami2019effective,
  title={An Effective Machine Learning Framework for Data Elements Extraction from the Literature of Anxiety Outcome Measures to Build Systematic Review},
  author={Goswami, Shubhaditya and Pal, Sukanya and Goldsworthy, Simon and Basu, Tanmay},
  booktitle={International Conference on Business Information Systems},
  pages={247--258},
  year={2019},
  organization={Springer}
}
@article{olorisade2019use,
  title={The use of bibliography enriched features for automatic citation screening},
  author={Olorisade, Babatunde Kazeem and Brereton, Pearl and Andras, Peter},
  journal={Journal of biomedical informatics},
  volume={94},
  pages={103202},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{alamri2015automatic,
  title={Automatic identification of potentially contradictory claims to support systematic reviews},
  author={Alamri, Abdulaziz and Stevensony, Mark},
  booktitle={2015 IEEE International Conference on Bioinformatics and Biomedicine (BIBM)},
  pages={930--937},
  year={2015},
  organization={IEEE}
}

@article{cohen2015automated,
  title={Automated confidence ranked classification of randomized controlled trial articles: an aid to evidence-based medicine},
  author={Cohen, Aaron M and Smalheiser, Neil R and McDonagh, Marian S and Yu, Clement and Adams, Clive E and Davis, John M and Yu, Philip S},
  journal={Journal of the American Medical Informatics Association},
  volume={22},
  number={3},
  pages={707--717},
  year={2015},
  publisher={Oxford University Press}
}

@inproceedings{goswami2019effective,
  title={An Effective Machine Learning Framework for Data Elements Extraction from the Literature of Anxiety Outcome Measures to Build Systematic Review},
  author={Goswami, Shubhaditya and Pal, Sukanya and Goldsworthy, Simon and Basu, Tanmay},
  booktitle={International Conference on Business Information Systems},
  pages={247--258},
  year={2019},
  organization={Springer}
}

@inproceedings{gotz2018supporting,
  title={Supporting systematic literature reviews in computer science: the systematic literature review toolkit},
  author={G{\"o}tz, Sebastian},
  booktitle={Proceedings of the 21st ACM/IEEE International Conference on Model Driven Engineering Languages and Systems: Companion Proceedings},
  pages={22--26},
  year={2018}
}
@article{oliver2015capacity,
  title={Capacity for conducting systematic reviews in low-and middle-income countries: a rapid appraisal},
  author={Oliver, Sandy and Bangpan, Mukdarut and Stansfield, Claire and Stewart, Ruth},
  journal={Health research policy and systems},
  volume={13},
  number={1},
  pages={23},
  year={2015},
  publisher={Springer}
}

@article{ghafari2012federated,
  title={A federated search approach to facilitate systematic literature review in software engineering},
  author={Ghafari, Mohammad and Saleh, Mortaza and Ebrahimi, Touraj},
  journal={International Journal of Software Engineering \& Applications},
  volume={3},
  number={2},
  pages={13},
  year={2012},
  publisher={Academy \& Industry Research Collaboration Center (AIRCC)}
}

@inproceedings{bekhuis2015prototype,
  title={A prototype for a hybrid system to support systematic review teams: A case study of organ transplantation},
  author={Bekhuis, Tanja and Tseytlin, Eugene and Mitchell, Kevin J},
  booktitle={2015 IEEE International Conference on Bioinformatics and Biomedicine (BIBM)},
  pages={940--947},
  year={2015},
  organization={IEEE}
}

@article{kitchenham2009systematic,
  title={Systematic literature reviews in software engineering--a systematic literature review},
  author={Kitchenham, Barbara and Brereton, O Pearl and Budgen, David and Turner, Mark and Bailey, John and Linkman, Stephen},
  journal={Information and software technology},
  volume={51},
  number={1},
  pages={7--15},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{olorisade2016critical,
  title={A critical analysis of studies that address the use of text mining for citation screening in systematic reviews},
  author={Olorisade, Babatunde K and de Quincey, Ed and Brereton, Pearl and Andras, Peter},
  booktitle={Proceedings of the 20th International Conference on Evaluation and Assessment in Software Engineering},
  pages={1--11},
  year={2016}
}

@article{sjoberg2005,
  title={A survey of controlled experiments in software engineering},
  author={Sj{\o}berg, Dag IK and Hannay, Jo Erskine and Hansen, Ove and Kampenes, Vigdis By and Karahasanovic, Amela and Liborg, N-K and Rekdal, Anette C},
  journal={IEEE transactions on software engineering},
  volume={31},
  number={9},
  pages={733--753},
  year={2005},
  publisher={IEEE}
}
@book{miles1994qualitative,
  title={Qualitative data analysis: An expanded sourcebook},
  author={Miles, Matthew B and Huberman, A Michael and Huberman, Michael A and Huberman, Michael},
  year={1994},
  publisher={sage}
}


@inproceedings{carver2013identifying,
  title={Identifying barriers to the systematic literature review process},
  author={Carver, Jeffrey C and Hassler, Edgar and Hernandes, Elis and Kraft, Nicholas A},
  booktitle={2013 ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={203--212},
  year={2013},
  organization={IEEE}
}
@inproceedings{kitchenham2009impact,
  title={The impact of limited search procedures for systematic literature reviews—A participant-observer case study},
  author={Kitchenham, Barbara and Brereton, Pearl and Turner, Mark and Niazi, Mahmood and Linkman, Stephen and Pretorius, Rialette and Budgen, David},
  booktitle={2009 3rd international symposium on empirical software engineering and measurement},
  pages={336--345},
  year={2009},
  organization={IEEE}
}

@inproceedings{molleri2016survey,
  title={Survey guidelines in software engineering: An annotated review},
  author={Moll{\'e}ri, Jefferson Seide and Petersen, Kai and Mendes, Emilia},
  booktitle={Proceedings of the 10th ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={1--6},
  year={2016}
}

@inproceedings{riaz2010experiences,
  title={Experiences conducting systematic reviews from novices’ perspective},
  author={Riaz, Mehwish and Sulayman, Muhammad and Salleh, Norsaremah and Mendes, Emilia},
  booktitle={14th International Conference on Evaluation and Assessment in Software Engineering (EASE)},
  pages={1--10},
  year={2010}
}
@article{brereton2007lessons,
  title={Lessons from applying the systematic literature review process within the software engineering domain},
  author={Brereton, Pearl and Kitchenham, Barbara A and Budgen, David and Turner, Mark and Khalil, Mohamed},
  journal={Journal of systems and software},
  volume={80},
  number={4},
  pages={571--583},
  year={2007},
  publisher={Elsevier}
}


@book{corbin2014,
  title={Basics of qualitative research: Techniques and procedures for developing grounded theory},
  author={Corbin, Juliet and Strauss, Anselm},
  year={2014},
  publisher={Sage publications}
}

@article{Kitchenham2002PrinciplesOS,
  title={Principles of survey research: part 5: populations and samples},
  author={Barbara A. Kitchenham and Shari Lawrence Pfleeger},
  journal={ACM SIGSOFT Software Engineering Notes},
  year={2002},
  volume={27},
  pages={17-20}
}
@article{Kitchenham2003PrinciplesOS,
  title={Principles of survey research part 6: data analysis},
  author={Barbara A. Kitchenham and Shari Lawrence Pfleeger},
  journal={ACM SIGSOFT Software Engineering Notes},
  year={2003},
  volume={28},
  pages={24-27}
}
@article{Kitchenham2007,
  title={Guidelines for performing Systematic Literature Reviews in Software Engineering},
  author={Barbara Kitchenham and S Charters},
  year={2007} 
}
@Book{Babar2009 ,
title={Systematic Literature Reviews in Software Engineering: Preliminary Results from Interviews with Researchers},
author={Muhammad Ali Babar et al.},
year={2009},
publisher={IEEE}
}
@Book{Wohlin2012,
title={Experimentation in Software Engineering: An Introduction},
author={Wohlin C, Runeson P, Höst M, Ohlsson MC, Regnell B, Wesslén A},
year={2012},
publisher={Springer Science & Business Media}

}
@Book{MORSE2000 ,
title={Designing funded qualitative research.},
author={JANICE M. MORSE},
url={http://www.qualitative-research.net/index.php/fqs/article/view/1428/3027},
year={2000},
publisher={https://journals.sagepub.com}
}

% -- Marcos ----

@inproceedings{imtiaz2013tertiary,
  title={A tertiary study: experiences of conducting systematic literature reviews in software engineering},
  author={Imtiaz, Salma and Bano, Muneera and Ikram, Naveed and Niazi, Mahmood},
  booktitle={Proceedings of the 17th International Conference on Evaluation and Assessment in Software Engineering},
  pages={177--182},
  year={2013}
}

@article{kitchenham2013systematic,
  title={A systematic review of systematic review process research in software engineering},
  author={Kitchenham, Barbara and Brereton, Pearl},
  journal={Information and software technology},
  volume={55},
  number={12},
  pages={2049--2075},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{hassler2014outcomes,
  title={Outcomes of a community workshop to identify and rank barriers to the systematic literature review process},
  author={Hassler, Edgar and Carver, Jeffrey C and Kraft, Nicholas A and Hale, David},
  booktitle={Proceedings of the 18th International Conference on Evaluation and Assessment in Software Engineering},
  pages={1--10},
  year={2014}
}





@article{ribeiro2018challenges,
  title={Challenges and pitfalls on surveying evidence in the software engineering technical literature: an exploratory study with novices},
  author={Ribeiro, Talita Vieira and Massollar, Jobson and Travassos, Guilherme Horta},
  journal={Empirical Software Engineering},
  volume={23},
  number={3},
  pages={1594--1663},
  year={2018},
  publisher={Springer}
}



@article{barn2014slrtool,
  title={Slrtool: a tool to support collaborative systematic literature reviews},
  author={Barn, Balbir and Raimondi, Franco and Athiappan, Lalith and Clark, Tony},
  year={2014},
  publisher={SCITEPRESS}
}

@article{al2017vision,
  title={Vision for SLR tooling infrastructure: Prioritizing value-added requirements},
  author={Al-Zubidy, Ahmed and Carver, Jeffrey C and Hale, David P and Hassler, Edgar E},
  journal={Information and Software Technology},
  volume={91},
  pages={72--81},
  year={2017},
  publisher={Elsevier}
}



@inproceedings{law2017crowdsourcing,
  title={Crowdsourcing as a tool for research: Implications of uncertainty},
  author={Law, Edith and Gajos, Krzysztof Z and Wiggins, Andrea and Gray, Mary L and Williams, Alex},
  booktitle={Proceedings of the 2017 ACM Conference on Computer Supported Cooperative Work and Social Computing},
  pages={1544--1561},
  year={2017}
}

@article{ramirez2018crowdrev,
  title={Crowdrev: a platform for crowd-based screening of literature reviews},
  author={Ramirez, Jorge and Krivosheev, Evgeny and Baez, Marcos and Casati, Fabio and Benatallah, Boualem},
  journal={arXiv preprint arXiv:1805.12376},
  year={2018}
}

@article{brown2014using,
  title={Using crowdsourcing to evaluate published scientific literature: methods and example},
  author={Brown, Andrew W and Allison, David B},
  journal={PloS one},
  volume={9},
  number={7},
  year={2014},
  publisher={Public Library of Science}
}

@article{mortensen2017exploration,
  title={An exploration of crowdsourcing citation screening for systematic reviews},
  author={Mortensen, Michael L and Adam, Gaelen P and Trikalinos, Thomas A and Kraska, Tim and Wallace, Byron C},
  journal={Research synthesis methods},
  volume={8},
  number={3},
  pages={366--386},
  year={2017},
  publisher={Wiley Online Library}
}



@inproceedings{nguyen2015combining,
  title={Combining crowd and expert labels using decision theoretic active learning},
  author={Nguyen, An Thanh and Wallace, Byron C and Lease, Matthew},
  booktitle={Third AAAI conference on human computation and crowdsourcing},
  year={2015}
}

@inproceedings{cranshaw2011polymath,
  title={The polymath project: lessons from a successful online collaboration in mathematics},
  author={Cranshaw, Justin and Kittur, Aniket},
  booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1865--1874},
  year={2011}
}

@inproceedings{mitchell2018coordinating,
  title={Coordinating advanced crowd work: Extending citizen science},
  author={Mitchell, Erica and Crowston, Kevin G and Oesterlund, Carsten},
  booktitle={51st Annual Hawai'i International Conference on System Sciences},
  year={2018}
}



@inproceedings{kitchenham2004evidence,
  title={Evidence-based software engineering},
  author={Kitchenham, Barbara A and Dyba, Tore and Jorgensen, Magne},
  booktitle={Proceedings. 26th International Conference on Software Engineering},
  pages={273--281},
  year={2004},
  organization={IEEE}
}




@inproceedings{marshall2015systematic,
  title={Systematic review toolbox: a catalogue of tools to support systematic reviews},
  author={Marshall, Christopher and Brereton, Pearl},
  booktitle={Proceedings of the 19th International Conference on Evaluation and Assessment in Software Engineering},
  pages={1--6},
  year={2015}
}

@article{marshall2018tool,
  title={Tool features to support systematic reviews in software engineering--a cross domain study},
  author={Marshall, Christopher and Kitchenham, Barbara and Brereton, Pearl},
  journal={e-Informatica Software Engineering Journal},
  volume={12},
  number={1},
  year={2018}
}



==> Image/Backup/discussion.tex <==
Previous research into SLR-related challenges has tended to focus on SLR activities related challenges rather than the root of these challenges that are the hallmark of this type of research\cite{imtiaz2013tertiary,carver2013identifying}
In our survey, we considered how communication
and automation approaches are used to support a number of different activities that researchers care about, such as learning and sharing with others, networking, and keeping up to date with new technologies and project activities. 

Our survey was answered by researchers who have conducted an SLR in the past 2 years in EBSE. When we designed our survey, we expected that this population may
and that we might see differences across the demographics
in the number and types of tools used and their
perceived benefits and challenges. Our expectations were
somewhat met—the respondents were skewed in the manner
we expected—but our analysis did not reveal

Our quantitative and in-depth analysis results showed that SLR authors have a diversity of challenges when conducting systematic reviews. It revealed that despite the common challenges of conducting SLRs, this process has other hidden corners that generates unknown new challenges, for which, many novice researchers are not well equipped or prepared, when starting a review. It also revealed how researchers employ different approaches to mitigate these challenges. We also discussed the challenges that prevent the researchers from employing existing Collaboration and automation solutions in their SLRs.

We seek to uncover challenges and opportunities in citizens involvement in the scientific research process.

It was evident from our findings that SLR-related challenges are embedded in a broader group of di  such as insufficient human resources, scarce research funding and insufficient collaboration channels for SLR community members. 
Previous research investigated the SLR-related challenges (Section~\ref{RelatedWorks}). 
With understanding these fundamental issues, we attempt to make the accounts of the survey participant research journey heard and make it beneficial to other novice and/or experienced researchers.

Even though the manual systematic review is prone to errors and it is time-consuming, however, reviewers have concerns regarding the accuracy and reliability of the automation techniques. For some tasks, humans are far more superior to the machines, whereas, in other tasks that require consistent iterations, machines outperform humans. In this regard, we believe future research should address human and machine collaboration through a cognitive computing system, to promote the collaboration between humans and machines for improving the performance of the machines.\newline 

The SLR community has witnessed a major paradigm shift in recent years in how researchers communicate and participate in this type of research. The new collaborations of researchers with third parties outside their SLR team, as well as utilizing technological artifacts, started to re-shape the SLR ecosystem. 
This study sheds more light on how researchers use different artefacts in their SLR experience.

Additionally, this study can be extended to commercial projects. Tools developers can review our findings (challenges and  solutions) and be motivated to focus on the real SLR's pain-points to develop more practical tools. In addition, they may utilize the solution strategies to develop new system.

Another important finding is that the researchers have concerns to adopting an automatic (e.g., crowdsourcing and machine learning) approach in conducting SLRs. We present that these concerns are related to the accuracy, security and the cost of such approches. view and examine this challenge from the perspective of scientific production, attribution and dissemination in massively authored research artefacts, bringing together the perspectives of researchers,citizens, editors and publishers so as to define models, processes and recommendations for crowdsourced SLR.


==> Image/Backup/doco.tex <==
% Effective software defect estimation can bring cost reduction and efficient resources allocation in software development and testing. Usually, estimation of defect-prone modules is based on the supervised learning of the modules at the same logical level. Various practical issues may limit the availability or quality of the attribute-value vectors extracting from the high-level modules by software metrics. In this paper, the problem of estimating the defect in high-level software modules is investigated with a multi-instance learning (MIL) perspective. In detail, each high-level module is regarded as a bag of its low-level components, and the learning task is to estimate the defect-proneness of the bags. Several typical supervised learning and MIL algorithms are evaluated on a mission critical project from NASA. Compared to the selected supervised schemas, the MIL methods improve the performance of the software defect estimation models.
% The dataset we use for training  set of 23,618 abstracts with titles were collected from 3 published SLRs, as part of a systematic review done by the McMaster University’s Evidence-Based Practice Center using TrialStat Corporation’s Systematic Review System 3 , a web-based software platform used to conduct systematic reviews. The initial set of abstracts was collected using a set of Boolean search queries that were run fo
% we describe the corpus (dataset) used to extract raw sentences and generate
% labeled sentences with event-types. Such sentences are used as training data for the
% event recognition technique we propose in the next section.



abstracts 



% Systematic literature reviews (SLRs) aim at analyzing and synthesizing research evidence, following accepted community guidelines, in response to postulated research questions. SLR process is highly cognitive, requiring acute human-judgment. Literature reviews can be time-consuming and tedious to complete.

% We evaluated our framework dataset along with its evaluation with human judgement.
% Finally, we present an exemplary task of security professional
% selection for bug bounty programs.


%by creating .... over 23,618 user-curated abstracts it was more than \textbf{x} time  faster than dedicated curators, and its output was of comparable quality. We reflect on the challenges and opportunities introduced by SLR\_PRO to inform the design of SLR curation systems that need subjective human judgments of papers.


% as sifting through thousands of citations to find relevant ones.
% Systematic literature reviews (SLRs) aim at analyzing and synthesizing research evidence, following accepted community guidelines, in response to postulated research questions. They are one of the most salient forms of publications in science and are the basis for evidence-based practices and even government policies. The SLR process is typically structured in phases, involving: (i) defining a goal; (ii) screening; (iii) analyzing; and (iv)  reporting the findings. The SLR process is highly cognitive, requiring acute human-judgment. For these reasons, it is no doubt, SLRs are very time consuming, become rapidly outdated, and are not easy to maintain. Accordingly, we investigate the emergence of cognitive computing and its impact on processes. Termed, ``cognitive process'' this new breed should augment current process technology (from structured to unstructured) with the rich and already mature advances in data curation, machine learning, context awareness as well as the crowd, and delivering this to end-users as natural and interactive digital assistance. In this paper, we explore this vision and present our initial findings applied in the context of the SLR use-case.
 
% With the ever increasing number of articles that are published everyday, conducting reviews become even more challenging.

% They are one of the most salient forms of publications in science and are the basis for evidence-based practices and even government policies. SLR process is highly cognitive, requiring acute human-judgment. For these reasons, it is no doubt, SLRs are very time-consuming, and are not easy to maintain. 
% With the ever increasing number of articles that are published everyday, conducting reviews become even more challenging.

% Hundreds of citation are screened to identify relevant studies with embedded answers to proposed research questions. 
% Recently, some studies have revealed that using machine learning and text mining methods to automatically identify relevant studies has the potential to improve the process by decreasing the workload in the screening phase.

% -- refere to web services ,... 

% In this work, we explore a decision support architecture to assist in the study selection process as high quality, low latency, and low-cost solution. We describe a framework to find the relevance of candidate studies to the systematic review research questions.
% This is a new way to find most relevant citations. 

% In addition we build upon such existing techniques, and validate it by experimenting on a large and comprehensive dataset form previously published systematic reviews. Our experiments provide insights on the use of feature extraction models that is domain-independent.

% \begin{table}
% \caption{Descriptive information for experimental datasets.}\label{table:datsets}
% \begin{tabular}{ p{0.2\textwidth}|p{0.15\textwidth}|p{0.15\textwidth}| c }
% \hline
% Datasets &  Candidate & Relevant & Research Questions \\
% \hline
% Wahono\cite{wahono2015systematic} &  2117 & 72 &\\
% Hall~\cite{hall2011systematic} &  2073 & 136 & \\
% Radjenovic~\cite{radjenovic2013software}& 13126 & 106 & \\
% \hline
% \end{tabular}
% \end{table}



% Figure~\ref{fig:Pipeline} illustrates a three-layer architecture to realize this vision. We start by leveraging (not reinventing) current process technology, including structured, unstructured and case management. We analyze this rudimentary layer with respect to: \emph{data}, \emph{tasks} and \emph{communication} capabilities. We then identify what \emph{enables} cognitive augmentation, and this depends on utilizing advances in machine-driven automation, human workers and most importantly reasoning and adapting. Cognitive processes must iteratively discover, learn and customize based on accumulated knowledge and experience. Finally, to the end-user cognitive processes means \emph{delivering} a digital administrative assistant (a ``humanoid''). It must support natural language interactions resembling the work practices of humans (providing guidance, advice, recommendation, contextualization and problem solving in decision making).



% This scenario, in particular, represents how cognitive support is enabled using a mesh of automated (e.g., algorithms, services, and AI). 
% One of the most labor-intensive yet critical phases is the planning phase. Focusing on this phase alone, we explore how cognitive support can be enabled to deliver several assistive components, working together to enable authors in performing reviews that are unbiased, systematic, inclusive, yet tractable in terms of effort and latency.


One of the most labor-intensive yet critical phases in SLR is the planning phase. Focusing on this phase alone, we explore how cognitive support can be enabled to deliver several assisting components, working together to enable authors in performing reviews that are unbiased, systematic, inclusive, yet tractable in terms of effort and latency. This scenario, in particular, represents how cognitive support is enabled using a mesh of automated (e.g., algorithms, services, and AI). The goal of the human workers in this scenario is both to conduct tasks along the way that require human intuition, as well as providing feedback for ongoing adaptation, such as input to reinforcement algorithms. At the human layer, that may be abstracted into the following components that feed into each other but can also be iterated as the authors (and algorithms) gain more insights of the outcomes of each phase: i) search, referring to setting the scope and identifying the relevant reviews; ii) annotate, the activity of labeling, filtering out and classifying scientific articles, and iii) synthesize, as the activity of extracting and deriving knowledge concerning the research question and overall analytical framework of the review.
In the following, we identify some of the relevant cognitive support areas for this scenario:\\



% Managing the endless amount of data from an ever-increasing number of SLRs is a challenge for most of the researchers. These datasets that are managed independently by research groups are often curated manually and consist of valuable information that can be used in future researchers. To mitigate this challenge, we propose using the Data Lake concept which al-
% lows storing all structured and unstructured data at any scale into a centralized
% repository. The data in the format of semi-structured data (CSV, JSON), un-
% structured data (documents) can be saved and used for advanced analytics in
% the application layer [32].

The inspiration behind our proposed approach is leveraging a similar approach to the word embedding's~\cite{mikolov2013distributed} model that represents words in a VSM. While general-purpose word embedding models often consider “words” as vectors, we have extended this idea to represent research any given corpus in a VSM. After encoding the given corpus(such as research question or the abstracts) into vectors, these VSMs are then used to calculate the similarity of the given pairs ( the research questions and list of abstracts) or passing through the classification models.   


% : The Universal Sentence Encoder encodes text into high dimensional vectors, this model is trained and optimized for greater-than-word length text, such as sentences, phrases or short paragraphs [6].

% : which comes in two variants, namely, Continuous Bagof-Words (CBOW) and Skip-Gram. [27]
% % \Indent:A pre-trained model on ConceptNetFootnote13 an open multilingual knowledge graph [40].
% \Indent: A previously fastText trained model on Wikipedia (2017),UMBC webbase corpus and statmt.org news with 16 billion words [3].
% \Indent: A publicly available word2vec model trained on Google News
% with about 3 million words and phrases [7].


%  After finding the top matching n-grams, the classifier would classify the reviews as relevant or irrelevant. The result then would be presented to the users in the interface. This layer enables researchers to call the SLR PRO APIs  based on their need and data, it also presets the insights that are embedded within the corpora. 

% After finding the top matching n-grams, the classifier would classify the reviews as relevant or irrelevant. The result then would be presented to the users in the interface.


% In this section, we present the architecture of our proposed framework to facilitate planning phase of systematic review. Fig~\ref{fig:Pipeline} illustrates the framework that is implemented in three tiers. In the following section, we provide details on how we leverage state-of-the-art technologies to build each tier of this framework: 
% Cognitive SLR is not about integrating AI into the process but augmenting current process technology with the vibrant and already mature advances in data curation, machine learning, and delivering this to SLR researchers as natural and interactive user interface and digital assistance.  To achieve this vision, we present the conceptual architecture of the SLR-PRO. Fig.~\ref{fig:Pipeline} presents the three-layer architecture of this system. We start by leveraging (not reinventing) the current process technology. We then analyze the initial layer ( service layer) with respect to: \emph{data}, \emph{tasks} and \emph{services} capabilities.

% The endless amount of data from an ever-increasing number of published systematic reviews and fragmented ownership of the curated data by independent research groups make it challenging to access the relevant data. To mitigate this challenge as well as save up the processing time when creating the vector spaces model for a given corpus, we propose using the Data repository which allows storing data at any scale into a centralized repository and be used for advanced analytics.
% We also introduce words similarity dataset for 
% and practitioners overcome this limitation.
% propose to Words Similarity Dataset.
% \subsubsection{Data Pre-Processing and Cleaning}

% \subsubsection{SLR Word Embeddings Learning}


% % Automation of this task is to find systematic reviews that answer the research question without manually translating research questions into search queries. Question answering systems have been in development since the 1960s [37]. For this task, a form of an automatic web-based question-answering system [38, 39] in which the answer to the review question is a systematic review, is most suitable.
% Even upon improving our query and finding relevant reviews, in many cases, it is still necessary to sift out irrelevant papers that are out of scope. A clear definition of the exclusion criteria is required to filter out irrelevant papers. The SLR-PRO machine-learning classifiers can be used to label articles as relevant and irrelevant that would help further refining the query (e.g., incorporating new keywords) as well as feedback into the refinement loop of the process.

% To make the dataset suitable for this experiment we added additional information such as SLR's research questions and SLR abstracts to the available dataset which originally contained information regarding screened included or excluded abstracts for 3 reviews.


==> Image/Backup/doco_v1.tex <==
% \documentclass[sigconf,review,anonymous]{acmart}
% \documentclass[11pt,a4paper]{article}
% \documentclass[sigconf,review,anonymous]{acmart}
% \documentclass[sigconf]{acmart}
% \documentclass{acmart}
% \documentclass[acmsmall,anonymous]{acmart}
% \settopmatter{printacmref=false} 
% \renewcommand\footnotetextcopyrightpermission[1]{}  
% \pagestyle{plain} 
% \usepackage{amsfonts}
% \usepackage{eqparbox}
% \usepackage{arydshln}
% \usepackage{multirow}
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{url}
% \newcommand\BibTeX{B{\sc ib}\TeX}
% \usepackage{footnote}
% \usepackage{graphicx}
% \usepackage{booktabs,colortbl}
% \usepackage{color, colortbl}
% \usepackage{rotating}
% \usepackage{subfigure}
% \usepackage{booktabs} 
% \usepackage{tabularx}
% \usepackage[utf8]{inputenc}
% \usepackage{multirow}
% \usepackage{rotating}
% \usepackage{pdflscape}
% \usepackage{color, colortbl}
% \usepackage{enumitem} 
% \usepackage[toc,page]{appendix}
% \usepackage{tcolorbox}
% \usepackage{dblfloatfix}
% \usepackage{amsfonts}
% \usepackage{titlesec}
% \usepackage{amsmath}
% \usepackage{fdsymbol}
% \usepackage[shortlabels]{enumitem} 
% \titlespacing*{\section}{0pt}{1.1\baselineskip}{\baselineskip}
% \titlespacing*{\subsection}{0pt}{1.1\baselineskip}{\baselineskip}
% \documentclass[sigconf,review,anonymous]{acmart}
% \documentclass[11pt,a4paper]{article}
%\documentclass[sigconf]{acmart}


% \begin{table}[!ht]
% \caption{Index Term Filter on IEEEXplore}
% \label{table:IndexTerm}
% \vspace{-0.3cm}
% \begin{tabular}{p{8cm}}
% \toprule
% \textbf{Term} \\
% \midrule
% \midrule
% computer aided instruction\\
% software engineering \\
% software development management\\
% data analysis\\
% project management \\
% Internet of Things \\
% software quality\\
% Internet \\
% learning (artificial intelligence)\\
% Big Data\\
% data mining\\
% mobile computing\\
% knowledge management\\
% medical computing\\
% program testing\\
% \arrayrulecolor{black}\bottomrule 
% \arrayrulecolor{black}\bottomrule 
% \end{tabular}
% \end{table}


 In which, we will construct an API knowledge graph to encode and evolve different APIs of publication databases; and with applying techniques from NLP, ML and Entity Recognition, we perform the required synthesis from natural language expressions, provided by the end users, to respond the user with proper answer.

% In this study we follow the design intelligence methodology and how might we humanize a machine-based interaction? 

% Expedite. Are you looking to free up time for your customers or the business so they can intervene in tasks that technology is not yet ready to handle?
% Perhaps they want to be part of those interactions because of the human value they bring to it, or the emotional value it delivers them.

% Leveraging data intelligence to expedite or replace rote, repetitive tasks, enables machines to free up humans to deliver their best value to your business. Consider this possible design intelligence enabler whenever your customers could use some time to perform more valuable tasks. Alright, now onto the next enabler. 
% Transform. When framing a design challenge around an organization, the people and its values were often looking for opportunities to transform the business. In this case, transform data intelligence you have on market opportunities or customer behavior into an input used to frame your organization's goals, and how you might achieve those. For our final enabler, discover, we can use any patters of needs uncovered by data intelligence to reveal new ways to make the human experience a better one. For example, if a wholly, new need is discovered, then it can be used to develop a new product or service, or they can identify the need for a new design solution. To get on a very personal level with your customers, these discoveries could proactively help those who may be in need of assistance before they reach out or complain. Lastly, these could guide them as they use your products. So they have less points of resistance. So the next time you have some valuable inputs for machine intelligence, design intelligently by asking yourself, if any one of these four enablers might drive a design that fulfills the need of your customers in a new or previously unimaginable way.

% observations from customers framed by those you've made by interviewing stakeholders. You've also been blessed with a data scientist to offer some new perspectives on your customers, product, and business. How do you incorporate that data intelligence into your insights and ideas? 
% That's right, it means just what it sounds like, you have data that serves as evidence for your design hypothesis.

% . Last but not least, this is a fantastic way to verify what may be most valuable to research and experiment further. 


%  The problem with this approach is that it absolutely ignores all kinds of other inputs. I call that data paralysis.


% If you hear from people that something you currently provide or represent in a concept, is hard to decipher, you might try humanizing the experience to further clarify it. 
% Results Based on qualitative analysis of XXX responses from researchers, we identified the potential for  

% \subsection{How Crowdsourcing can be used in conducting an SLR?}
% Crowdsourcing enables one to leverage on the intelligence and wisdom of potentially large groups of individuals toward solving problems. Common problems approached with crowdsourcing are labeling images, translating or transcribing text, providing opinions or ideas, and similar - all tasks that computers are not good at or where they may even fail altogether. The introduction of humans into computations and/or everyday work, however, also poses critical, novel challenges in terms of quality control, as the crowd is typically composed of people with unknown and very diverse abilities, skills, interests, personal objectives and technological resources. This survey studies quality in the context of crowdsourcing along several dimensions, so as to define and characterize it and to understand the current state of the art. Specifically, this survey derives a quality model for crowdsourcing tasks, identifies the methods and techniques that can be used to assess the attributes of the model, and the actions and strategies that help prevent and mitigate quality problems. An analysis of how these features are supported by the state of the art further identifies open issues and informs an outlook on hot future research directions.

% S27&Any small details from your literature can become useful and it is easier if you start recording them at the beginning. Take a few days and make a list of everything you can extract from the literature into spreadsheet. is for me the key! \\
% S31& Also, different search engines give different results. For mine web of science found way more non-English articles than GS. And different parts of the world use different terms for similar ideas sometimes.\\
% S37&Find a way to keep organized during the different stages of the process so you can keep track of which articles fit your research question. Since you will be searching through thousands, this is essential\\

--- Reasoning 
% size of the data that has to be analyzed  Furthermore, the existing analytical tools can help the authors to generate visual analytic reports, and perform the analytical tasks quicker.
-- reasoning 2
% However, this requires a literature review for finding relevant secondary studies, prior to starting the SLR.
---reasoning 3
% This indicates another possibility that reviewers would not be aware of alternative that exists  for conducting the task in a more productive and efficient way.  
% The responds show that even though they reported high level of challenges for conducting the tasks.
% But, they reported that they have done the task manually. 

% \begin{itemize}
% \item Problems related to SLR researchers, including level of experience in conducting SLR; 
% \item Problems related to study scope, including the size of the study and the topic;
% \item Problems related the tools, including the absence of efficient support tools;
% \end{itemize}
% \begin{itemize}
% % Reviewers' level of experience in the topic of SLR (or in conducting SLRs); 
% % Would the level of domain knowledge significantly affect the user's search behaviour?
% \item The authors' solution awareness of the alternative ways for facilitating SLR process affect the  ; 
% \item The scope of the SLR study;
% % \item Adapting the best practices/guidelines;
% % \item level of usage of SLR support tools;
% %Relatively high level of experience/capability of respondents and their teams in the conducting SLR;
% \end{itemize}

% \begin{itemize}
% \item Following best practice  in addition to the SLR guidelines;
% \item Employing SLR tools and platforms that (semi-)automate some of the tasks;
% \item Seeking expert assistance to perform the tasks that require domain knowledge;
% \item Sharing the knowledge and experience about the solutions for a more sufficient SLR process;
% \end{itemize}

& It is necessary to conduct a pilot study before the actual study to test the protocol and apply the changes if it's required;\\
& 1. Keep organized during different stages of the process so you can keep track of which articles fit your research question and note all search details, even those that seem unnecessary to note.\\
& 2. Make regular backups and copies AND prevent duplicates where you can use alias/links.\\
&3. It is necessary to conduct a pilot study before the actual study to test the protocol;\\
&  4.  When designing data extraction forms pick a couple of relevant studies to pilot the data extraction forms on, so you know you are extracting all the relevant info\\
& 5. Test your search query to find the papers. Use indicator papers which should be picked up.\\
& 6. Do not 100\% rely on earlier reviews, they might have excluded a lot of relevant research.\\
& 7. Google Scholar searches the full-text, while other standardized databases are limited to only abstract, title and keywords. If your search term is not a major buzzword, you will get more hits with GS.\\
& 7. Plan your analysis, select 30 papers, do all your analysis on those 30 papers. You can't plan to cover all the topics before you start analyzing.\\
& 8. Perform robust inter-coder reliability\footnote{inter-coder reliability refers to the extent to which two or more independent coders agree on the coding of the content of interest with an application of the same coding scheme.}.\\
& 9. Keep a record of all modifications to the code/tagging book that you make.\\
& 10. Think carefully about the classification scheme. Also the data you will extract from the papers. Test it with a subset of papers and refine the method.\\
 & 11. Keep URLs, DOIs, titles, and abstracts in your extracted spreed sheet for the future reference.\\
& 12. Know when the cutoff is for papers being archived -(before all papers appear from the previous year).\\
& 13. A well-organized spreadsheet, Be comprehensive when recording the data, this would help with analysis.\\
& 14. keep detailed notes on the exact search queries you run and in what databases.\\
& 15. Get into the different algorithms of literature search databases. The same search term combination will be used differently. Do a pre-search where you evaluate search terms and portals.\\
& 16. I would suggest setting cut-off for what you will include new papers. If you don't set a cut off boundary, it is way too easy to get caught in the 'I'll just include this one more brand new trap.\\
& 17. Don’t let the paper stay too long after review to avoid needing to add too many recent papers.\\

\human  
& 1. Consider working with an information specialist to help design a comprehensive and efficient search strategy\\
& 2. librarians can advise on appropriate databases and help design search strategies.\\ 
& 3. Do not try to do it alone."Teamwork"\\
& 4. I assign to my grad students.\\
& 5. Let the 1st \& 2nd round of inclusion decision done by 2 ppl.\\
& 6. it's good to plan ahead and know what sort of information readers and reviewers will be expecting (e.g. date of search, inclusion criteria etc.), check the interpretation of data extraction from cross reviewers so data is being extracted in the same way\\
& 7. Definitely consult potential end-users of the review of how they envision using it, what kinds of questions will they ask of it? What level of risk and uncertainty is acceptable?\\ 
& 8. Get your protocol reviewed externally if at all possible. You could get some really useful feedback.\\ 
& 9. Include some review experts in your team (or have some on hand to ask questions of) if possible too. Same with topic experts for those tricky inclusion decisions.\\


\textit{\textbf{Tools}} &\\
& 1. use software for storing articles, notes, coding, etc \textit{DevonThink} .\\
& 2. Use reporting system is useful, also for making figures and documenting \textit{Roses}.\\
& 3. use tools that are empowered with machine learning to organize large sets of citations.\textit{colandr}.\\
& 4.  Use software to manage the reference. It's saved me so many times. \textit{DistillerSR}\\
& 5. Use "Endnote" multi-user so multiple people can work on the same archive Record papers will null returns so you know you searched them!\\
& 6. Use systematic review software like @Covidence  to do your screening. Makes all the difference and saves loads of time.\\
& 7. Be mindful of critiquing the quality assessment tool to make sure it i) covers all issues of bias relevant to study designs included, ii) that it assesses biases rather than reporting issues, these are guides;\\

% \item eporting system is useful, also for making figures and documenting Roses.\\
% \item use tools that are empowered with machine learning to organize large sets of citations\\
% \item Use systematic review software like @Covidence to do your screening. Makes all the difference and saves loads of time.\\
% \item Be mindful of critiquing the quality assessment tool to make sure it i) covers all issues of bias relevant to study designs included,ii) that it assesses biases rather than reporting issues, these are guide\\

%  Very important

\begin{table*}[t]
\small
\caption{Survey Questions}
\label{table:SurveyQuestions}
\vspace{-0.3cm}
\begin{tabular}{p{0.5cm}|p{0.5cm}|p{15cm}}
\toprule
\textbf{\#} & \textbf{RQ}&\textbf{ Survey Question}\\
\toprule
&&\hspace{100pt}\textit{\textbf{General Question}}\\
\arrayrulecolor{black!20}\midrule
Q1 &Dem& Please answer the following questions about your experience in conducting SLR\\
1.1 && How many SLRs have you conducted?\\
1.2 && How many reviewers were involved in conducting these reviews? \\
1.3 && How long did it take to complete these reviews on average? \\
1.4 && What was the research area of these SLRs? \\
1.5 && What was your status when conducting the SLR(s)? (e.g., Ph.D student) \\
\arrayrulecolor{black}\midrule
&&\hspace{100pt}\textit{\textbf{Planning Phase}}\\
\arrayrulecolor{black!20}\midrule
Q2&& Please choose options that express your experience in performing following SLR tasks:\\
 2.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
 2.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
\arrayrulecolor{black!5}\midrule
T2.1&&\hspace{4pt}Finding previous secondary studies (e.g., SLRs)  \\
T2.2&&\hspace{4pt}Defining research questions \\
T2.3&&\hspace{4pt}Defining study search strategy (e.g., what databases to search, defining the search keywords)\\
T2.4&&\hspace{4pt}Defining data collection method (e.g. data extraction template)\\
\arrayrulecolor{black!5}\midrule
Q3&RQ1&Please describe challenges you faced while performing any tasks related to these phase of SLR.\\
Q4&RQ2&Please describe if you developed any solution or work-around to overcome the challenges of conducting these tasks.\\
Q5&RQ2&If you used tools or platforms for conducting these tasks, what did you like or dislike about them? If you didn't use any tool( due to its limitations) what possible solution do you wish available or analogous to tools in other fields?\\
Q6&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
% \arrayrulecolor{black}\midrule
% &&\hspace{100pt}\textit{\textbf{Conducting Phase}}\\
% \arrayrulecolor{black!20}\midrule
% Q7&&Please choose options that express your experience in performing following SLR tasks:\\
%  7.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
%  7.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
% \arrayrulecolor{black!5}\midrule
% T7.1&&\hspace{4pt}Building the search queries for each database\\
% T7.2&&\hspace{4pt}Retrieving and storing retrieved studies\\
% T7.3&&\hspace{4pt}Applying inclusion and exclusion criteria to filter studies\\
% T7.4&&\hspace{4pt}Screening titles and abstracts\\
% T7.5&&\hspace{4pt}Assessing the quality of the remaining studies \\
% T7.6&&\hspace{4pt}Extracting data from selected studies \\
% T7.7&&\hspace{4pt}Annotating and tagging for specific data categories (e.g.,PICO)\\
% \arrayrulecolor{black!5}\midrule
% Q8&RQ1&Please describe challenges you faced while performing these tasks related.\\
% Q9&RQ2&Please describe any solution or work-around you developed to overcome these challenges\\
% Q10&RQ2&If you used tools or platforms for conducting these tasks, what did you like or dislike about them?If you didn't use any tool( due to its limitations) what possible solution do you wish available or analogous to tools in other fields?\\
% Q11&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
% \arrayrulecolor{black}\midrule
% &&\hspace{100pt}\textit{\textbf{Reporting Phase}}\\
% \arrayrulecolor{black!20}\midrule
% Q12&& Please choose options that express your experience in performing following SLR tasks:\\
%  12.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
%  12.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
% \arrayrulecolor{black!5}\midrule
% T12.1&&\hspace{4pt}Documenting the findings\\
% T12.2&&\hspace{4pt}Analyzing and synthesizing collected data\\
% T12.3&&\hspace{4pt}Writing the report\\
% \arrayrulecolor{black!5}\midrule
% Q13&RQ1&Please describe challenges you faced while performing any tasks related to this phase.\\
% Q14&RQ2&Please describe any solution or work-around that you developed or aware of, to overcome these challenges.\\
% Q15&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
% \arrayrulecolor{black}\midrule
% &&\hspace{100pt}\textit{\textbf{Updating SLRs}}\\
% \arrayrulecolor{black!20}\midrule
% Q16&RQ1&Have you ever been involved in updating an existing SLR, could you please describe the pain points you found in this process?\\
% Q17&RQ2&Please describe your thoughts on improving the SLR-updating process to be a more feasible and less time-consuming process.\\
\arrayrulecolor{black}\bottomrule 
% \arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table*}

% \begin{figure}[h]
% \caption{Applied Filters to IEEEXplore}
% \label{fig:TermIndex}
% \includegraphics[width=7.5cm]{Image/TermIndex.pdf}
% \end{figure}
% \subsection{Data Collection}



\begin{table}[h]
\small
\caption{Most Popular Tools}
\label{table:Tools}
\vspace{-0.3cm}
\begin{tabular}{p{3.5cm}|p{1.5cm}}
\toprule
\textbf{Tools}&\textbf{Frequency}\\
\toprule
MS Excel	&28\\
Digital Libraries Search Tool	&22\\
Endnote	&8\\
MS Word	&6\\
Zotero	&6\\
Google Scholar	&5\\
Nvivo	&4\\
Google doc	&3\\
Jabref	&3\\
Mendeley	&3\\
QDALite	&3\\
Acrobat Adobe	&2\\
Dropbox	&1\\
Grammarly	&1\\
Latex( Overleaf)&1\\
PowerBI	&1\\
Tableau	&1\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table}


\subsection{Level of Challenges for SLR Tasks}
We asked the participants to select the level of difficulty for each tasks that they encountered when conducting SLR. Figure~\ref{fig:ChallengeLevel} presents the level of these challenges for main SLR tasks. The data points present number of participants who select the task either as time-consuming or complicated. As shown in this Figure, tasks related to the planning phase, are generally rated more challenging. This trend applies to both senior and novice (Ph.D. students) researchers. As one would expect, in the planning phase, novice researchers have more challenges in defining the study scope. However, "selecting the relevant keywords" was described as the most challenging task for both research groups.\\ "Composing search queries for digital libraries" was rated the second most time-consuming task by Ph.D. students. while "Defining the data collection method" was more of a difficult task for senior researchers. The data shows that screening abstracts is a labor-intensive task, mostly because of large number of irrelevant papers retrieved from digital libraries. However, some comments show that the study topic and scope have a direct effect the level of this difficulty. Also, data shows that some participants overcome this challenge by increasing the number of people who contribute to perform this task. One of the participants mentioned: "I get help from undergraduate students for screening the abstracts.". According to the survey outcome, data extraction is also one of the most challenging part SLR process. One mentioned: "I believe defining the data extraction template is one of the most complex steps.". Some suggest that to avoid deconstructing the data extraction rules. The task of defining "data-extraction-template" should be done when "initial paper screening" is concluded and more information is available about the characteristics of the included studies. Some novice researchers also mentioned that relevant SLRs ' method for data extraction and synthesis, could be helpful to define the data extraction practice, Yet, finding relevant SLRs is a challenging task by itself. The survey participants rated the "data synthesis" as the most complex task in the final phase of SLR. The survey participants believe that being organized and keeping records of all the findings is the key to mitigating the difficulties of this task.\\


\begin{table}[h]
\small
\caption{Main Reasons of the Challenges}
\label{table:ChallengesClass}
\vspace{-0.3cm}
\begin{tabular}{p{1cm}|p{6cm}}
\toprule
\textbf{\#}&\textbf{Challenges}\\
\toprule
Group1 & Problems related to SLR researchers, including their level of experience in conducting SLRs and their familiarity among the study topic;\\ 
\arrayrulecolor{black!20}\midrule
Group2 & Problems related to the tools and technologies, including the absence of support automation mechanisms, as well as limitations of the existing tools;\\
\arrayrulecolor{black!20}\midrule
Group3 & Problems related to the study scope, including the study size as well as the topic of the study;\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table}


Here, we present some of the comments of the participants to support this assumption. A senior researcher mentioned that "I didn't have much of a difficulty in defining the study scope.". While a Ph.D. student commented that "I don't know how extensive the review should be. For me, this is the most challenging component." Another Ph.D. student mentioned: " When I know a research field, I can easily decide what studies I will be looking for to include. But again, this requires knowing the field very well. But for the new fields, it is so difficult to define the study scope.". 



While the iterative tasks (such as composing different search queries for digital libraries) have been rated high challenging among both groups of the participants. while 


"Defining the SLR scope This is the fundamental phase and I guess the more experience you are the easier it gets. down the line, it involves a lot of manual efforts, but definitely have to seek for a second opinion on the search criteria 
Zotero to retrieve studies from google scholar, endnote to manage the files, I wish it was easier to tag the full-text, such as highlighting some data by default ( such as pico)  
"The tools are good helps, however I don't know the level of their accuracy, can't trust them , unless the tool is tested and the reviews are available."



In summary, we should highlight that in almost all above studies, discussions are among a specific task or towards finding only SLR challenges. Yet, in this study, we are systematically gather and analyze information from SLR authors and discuss the workarounds that they employ individually to overcome SLR's challenges. Also, we investigate the exiting concerns that researchers have in adopting machine and human computation techniques to automate part of this process.

Achieving a deeper understanding of how media shape this participatory culture will guide tool designers and provide recommendations for how individual researchers, teams, and communities should use the media effectively. In the next section, we describe a survey we designed to investigate this topic.



\begin{table*}[h]
\small
\caption{Top Rated Challenges Among SLR Tasks}
\label{table:Challenges}
\vspace{-0.3cm}
\begin{tabular}{p{0.5cm}|p{12cm}}
\toprule
\textbf{\#}&\textbf{Challenges}\\
\toprule
% &\hspace{100pt}\textbf{Search Task}\\
&\textbf{Study Search}\\
\arrayrulecolor{black!20}\midrule
1& Inconsistent use of terms and keywords by the authors across different disciplines; This makes it difficult to compose the search queries and make sure the retrieved studies are relevant;\\
2& Digital libraries have limitation on executing complex search queries; Therefor, it is required to break down the queries and run them in the simpler formats and merge the results of all the queries;\\
3&Each digital library works with a specific form of \textit{Boolean} search queries; Therefore the search queries should be modified and applied to each of them; which is a time-consuming process;\\
4&Digital libraries are unable to download the search result when the dataset is large; and there is a chance that some studies are missed in this transition;\\
5&Reproducing the search results is not consistent, and it depends on the point of time of running the search query;\\
6&Defining the search criteria requires a high level of domain knowledge; therefore it is taking time to find all the relevant keywords and terms to define a comprehensive search;\\
7&The search results usually saturated with irrelevant studies and finding duplicates is very time-consuming and requires a lot of manual inspections;\\
8& Some digital libraries have limit times for running search queries and when reaching the limitation has to wait for the next time to run the queries;\\ 
9&Digital libraries' APIs are not designed for SLR searching process and can't be easily used as a alternative to the manual search;\\
10& Most of digital libraries do not search full text and search fields are limited; It is easy to miss some studies due to this limitation;\\
% 9&Different versions of full-text is ain different libraries& \\
\arrayrulecolor{black!30}\midrule
&\textbf{Defining the Study Scope}\\
\arrayrulecolor{black!20}\midrule
1& To ensure that undertaking a new SLR is required it is required to find previous relevant systematic reviews or mapping studies. It is not possible to locate studies based on the study methodology, and this makes it time-consuming and prone to errors to search and find them;  \\
2&Composing clear research questions and define the objectives is one of the most prolong tasks in SLRs and required domain experts input and advises;\\
3& When the SLR's topic is new, defining the study scope and size of the study becomes even more difficult;\\
4&Classification scheme and data extraction template are difficult to define, specially for novice researchers; It requires many iterations of modification to assure that the template is inline with study's objectives and would extract all the required data;\\
\arrayrulecolor{black!30}\midrule
&\textbf{Paper Screening (e.g., excluding irrelevant studies)}\\
\arrayrulecolor{black!20}\midrule
1& It is difficult to locate the studies' methodology (systematic reviews ,comparative analyses, surveys, or interviews) in the selected studies ; this is critical for applying inclusion and exclusion criteria to select  candidate studies; Sometimes it is required to screen "Introduction" or further through the study to find this information;\\
2& Quality assessment is a complicated task and prone to human errors and personal judgments;\\
3&The result of the search is usually imbalanced with majority of the irrelevant studies; To provide a transparent study, it is required to keep tracks of the reasoning for excluding all these studies, it is time-consuming to fill up the forms and record them in an accessible way among the team of authors;\\
4&The full text of the studies are not easily accessible; Limited access to these documents is causing issues for the SLR reviewers; They constantly need to connect to the university libraries ' portal to access the latest version of the papers; otherwise, the purchasing costs is not feasible;\\ 
5&The abstracts screening is not limited to the abstracts only; in some cases the abstracts don't contain enough information for making decision to include a paper; it is very time-consuming to read the entire papers and find out they are not relevant;\\
6& Screening a large number of mostly irrelevant studies is one of the most intensive tasks of all;\\
\arrayrulecolor{black!30}\midrule
&\textbf{Data Extraction and Synthesising}\\
\arrayrulecolor{black!20}\midrule
1&The fact that authors use ambiguous terms to express the same concept makes the data extraction task laborious, time-consuming and prone to errors;\\
&Journals are not following the same structures to present Metadata information; This makes the Metadata extracting time-consuming; \\
3&The results of some studies are not clearly defined and it is required to repeat the paper screenings to find the study objectives and results;\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table*}




\begin{table}[h]
\small
\caption {Characteristic of the Solutions}
\label{table:Solutions}
\vspace{-0.3cm}
\begin{tabular}{p{0.75cm}|p{6.5cm}}
\toprule
\textbf{\#}&\textbf{Solutions}\\
\toprule
Data Stores& Following the best practice (e.g.,published SLRs) in addition to the SLR guidelines when conducting an SLR;\\
\arrayrulecolor{black!20}\midrule
Tools& Employing SLR tools and platforms to automate the tasks, speed up the process by reducing the manual work;\\
\arrayrulecolor{black!20}\midrule
People& Seeking expert's advice and utilize their domain knowledge in conducting the tasks;\\
\arrayrulecolor{black!20}\midrule
& Sharing knowledge and experience with other members of the SLR community, and inform them about available and alternative solutions;\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table}


\begin{table*}[h] 
%  fix position for table [!hp]
\small
\caption{Notes to researchers who conducting SLR for the first time}
\label{table:Solutions}
\vspace{-0.3cm}
\begin{tabular}{p{15cm}}
\toprule
\begin{itemize}
\item It is necessary to conduct a pilot study before starting SLR study.This is to test the protocol and apply changes if it's required.
\item It is also critical to pilot test data extraction template with a couple of relevant studies to make sure that all the required information is extracted base on the template;
\item Performing robust inter-coder reliability is also essential for tagging and data extraction task.\footnote{inter-coder reliability refers to the extent to which two or more independent coders agree on the coding of the content of interest with an application of the same coding scheme.}.
\item Search queries should be tested by using indicator papers; if the search criteria is defined properly this gold examples should appear in the search results.
\item It is necessary to keep records on the exact search queries. Digital libraries have an archiving process; this process defines the time that they release all the publications from the previous year. Therefore it is important to also keep notes on the query execution time.
\item Keeping records of all modifications to the code/tagging schemes is also necessary; and will be critical when there is a large set of studies;
\item Everyday new studies are published, hence setting a cut-off time for including new papers would help avoiding being caught in the trap of "one more brand new paper!".
\item The details about all the studies should be recorded specially the reason for excluding them.
\item Due to the high number of papers published every day, the data and findings can become obsolete quickly, therefore its is necessary that the result is published as soon as possible to avoid needing to add many recent papers and updating the results.
\item Some digital libraries provide searching through full-text search ( e.g., Google Scholar) while others are just limited to the abstract and title search, the chance is higher to get more hits with the first group of the search engines.
% \item Machine learning techniques can be used as a baseline to find related keywords.
% \item possible way is to rely on NLP to summarize text and check sentences structure and grammar when writing report.
% \item Crowds can be helpful in tagging the papers or screening the abstract for finding the topics.
% \item I guess distributing tasks between a larger group of people can reduce the deadlock, however
% \item Since the reporting phase relies on the authors' deductions and reasoning it would be hard to employ automation
\end{itemize}
% \arrayrulecolor{black}\bottomrule
\end{tabular}
\end{table*} 


% \begin{itemize}
% \item SLR researchers issues; 
% \item Coordination and collaboration difficulties;
% % \item Barriers to community building and participation;
% \item Study scope and topic hurdles;
% \item Content and knowledge management;
% \item SLR tools affordance and accessibility; % \item Automation techniques adoption concerns;
% \end{itemize}


% (i) \textbf{Unfamiliarity with the SLR topic} negatively impacts authors' efficiency in performing relevant tasks;\\ 
% (ii) \textbf{Awareness of the current solutions and tools} and workarounds would help reducing the challenges.\\


\begin{table*}
\small
\caption{Survey Questions}
\label{table:SurveyQuestions}
\vspace{-0.3cm}
\begin{tabular}{p{0.5cm}|p{0.5cm}|p{15cm}}
\toprule
\textbf{\#} & \textbf{RQ}&\textbf{ Survey Question}\\
\toprule
&&\hspace{100pt}\textit{\textbf{General Question}}\\
\arrayrulecolor{black!20}\midrule
Q1 &Dem& Please answer the following questions about your experience in conducting SLR.\\
1.1 && How many SLRs have you conducted?\\
1.2 && How many reviewers were involved in conducting these reviews? \\
1.3 && How long did it take to complete these reviews on average? \\
1.4 && What was the research area of these SLRs? \\
1.5 && What was your status when conducting the SLR(s)? (e.g., Ph.D student) \\
\arrayrulecolor{black}\midrule
&&\hspace{100pt}\textit{\textbf{Planning Phase}}\\
\arrayrulecolor{black!20}\midrule
Q2&& Please choose options that express your experience in performing following SLR tasks:\\
 2.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
 2.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
\arrayrulecolor{black!5}\midrule
T2.1&&\hspace{4pt}Finding previous secondary studies (e.g., SLRs)  \\
T2.2&&\hspace{4pt}Defining research questions \\
T2.3&&\hspace{4pt}Defining study search strategy (e.g., what databases to search, defining the search keywords)\\
T2.4&&\hspace{4pt}Defining data collection method (e.g. data extraction template)\\
\arrayrulecolor{black!5}\midrule
Q3&RQ1&Please describe challenges you faced while performing any tasks related to these phase of SLR.\\
Q4&RQ2&Please describe if you developed any solution or work-around to overcome the challenges of conducting these tasks.\\
Q5&RQ2&If you used tools or platforms for conducting these tasks, what did you like or dislike about them? If you didn't use any tool( due to its limitations) what possible solution do you wish available or analogous to tools in other fields?\\
Q6&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table*}


% This may indicate that at least 60 percent of our respondents develop for the Web.
% \section{Results}
% In this section we present the study's results. First, we provide an overview of the demographics, followed by the answers to the research questions.
% , then we discussion and recommendations, and a review of the potential threats to validity.
% \section{The Challenges Researchers Face When Conducting SLRs}

p36: data extraction requires a lot of time and concentration and the template may change after some iteration, due to findings in the articles 

p17:
for extracting data we used excel sheets in addition to highlighting text using adobe acrobat. we referenced the parts of the paper that related to specific codes and stored files in folders that contained families of papers (e.g., a folder for papers discussing specific quality control method) and within the folder we coded the file names to be easily referenced in the excel sheet 


% \begin{table}
% \small
% \caption{SLR Search Problems}
% \label{table:Study search}
% % \vspace{-0.3cm}
% \begin{tabular}{p{0.5cm}|p{6cm}|p{1cm}}
% \toprule
% \textbf{}&\textbf{Problems}&\textbf{\#Reports}\\
% \toprule
% 1& Inconsistent use of terms and keywords by the authors across different disciplines makes it difficult to compose the search queries;&25\\
% 2&Digital libraries have limitation on executing complex search queries; Therefor, it is required to break down the queries and run them in the simple formats and merge the results;20\\
% 3&Each digital library works with a specific form of Boolean search queries; Therefore, the search queries should be modified and applied to each of them, that makes it is time-consuming;&15\\
% 4&Digital libraries are unable to download the search result when the dataset is large; and there is a chance that some studies are missed in this transition;&10\\ 
% \arrayrulecolor{black}\bottomrule 
% \end{tabular}
% \end{table}

% \begin{table}
% \small
% \caption{SLR Search Problems}
% \label{table:Study search}
% % \vspace{-0.3cm}
% \begin{tabular}{p{0.5cm}|p{6cm}|p{1cm}}
% \toprule
% \textbf{}&\textbf{Problems}&\textbf{\#Reports}\\
% \toprule
% 1& Inconsistent use of terms and keywords by the authors across different disciplines makes it difficult to compose the search queries;&25\\
% 2&Digital libraries have limitation on executing complex search queries; Therefor, it is required to break down the queries and run them in the simple formats and merge the results;20\\
% 3&Each digital library works with a specific form of Boolean search queries; Therefore, the search queries should be modified and applied to each of them, that makes it is time-consuming;&15\\
% 4&Digital libraries are unable to download the search result when the dataset is large; and there is a chance that some studies are missed in this transition;&10\\ 
% \arrayrulecolor{black}\bottomrule 
% \end{tabular}
% \end{table}


% We also asked the respondents to share the details of challenges they face for any related task through open-ended text questions. Respondents either elaborated on the challenges mentioned above or informed us about other challenges they experienced.

% \begin{table}
% \small
% \caption{Test of Independence between Different Demographic Factors in the Survey}
% \label{table:Demographics}
% % \vspace{-0.3cm}
% \begin{tabular}{p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.5cm}}
% \toprule
% \textbf{}&\textbf{SLR Span}&\textbf{Team Size}&\textbf{SLR Nbrs}&\textbf{Experience}\\
% \toprule
% \textbf{SLR Span}&&$\rho$=0.4&$\rho$=-0.63&kw=\\
% \textbf{Team Size}&&&$\rho$=-0.76&kw=\\
% \textbf{SLR Nbrs}&&&&kw=\\
% \arrayrulecolor{black}\bottomrule 
% \end{tabular}
% \end{table}


The solutions provided by the participants have 3 main aspects:  Fig~\ref{fig:Solutions} presents the characteristic of the strategies used by participants to overcome challenges.\\
\begin{figure}[h]
\centering
\caption{Characteristic of the strategies used by participants to overcome challenges} 
\label{fig:Solutions}
    \includegraphics[width=7.5cm]{Image/Solution.pdf}
\end{figure}

% \subsection{Survey Responds}

% As shown in Fig~\ref{fig:SurveyDistribution},
% \begin{figure}[h]
% \caption{Survey Distribution and Response}
% \label{fig:SurveyDistribution}
% \includegraphics[width=7.5cm]{Image/SurveyDistribution.pdf}
% \end{figure}
% \begin{figure*}[h]
% \caption{Summary of the Findings}
% \label{fig:Findings}
% \includegraphics[scale=1]{Image/Findings.pdf}
% \end{figure*}
% the findings of this survey we categorized the findings into 3 categories 

% \begin{figure*}[h]
% \centering
% \caption{Notes to researchers conducting SLR for the first time} 
% \label{fig:NoteToNovice}
% \includegraphics[width=15cm]{Image/NoteToNovice.pdf}
% \end{figure*}


\begin{table}
\small
\caption{Test of Independence between Different Demographic Factors in the Survey}
\label{table:Demographics}
% \vspace{-0.3cm}
\begin{tabular}{p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.5cm}}
\toprule
\textbf{}&\textbf{SLR Span}&\textbf{Team Size}&\textbf{SLR Nbrs}\\
\toprule
\textbf{SLR Span}&&$\rho$=0.4&$\rho$=-0.63\\
\textbf{Team Size}&&&$\rho$=-0.76\\
\textbf{SLR Nbrs}&&&\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table}


They believe that being organized and keeping records of all the findings from the beginning is the key to mitigate the difficulties of this task. Next we summarize the specific problems raised for individual tasks and also how authors compromise performing the tasks because of these challenges. 

% (iv) Question related to desired features that the reviewers like to have them in SLR tools;\newline  
% (v) Question related to the concerns of adopting automation techniques in SLR process;\\

% Table~\ref{table:SurveyQuestions} presents the survey questions along with a mapping to the research questions(RQs).\\ 

In addition to this group of candidate, we added the first authors of SLR studies from our previous literature review.

We do not present the full survey questionnaire here due to space limitations, but Table~\ref{table:SurveyQuestions} presents part of the questionnaire to emphasize the reasons of including these questions by presenting the mapping between the research questions and the survey questions.\\

 \textit{It was included all manual efforts and it is time consuming to analyze the data and formulate the findings in an easy to digest way. sometimes we were obliged to hold long discussion sessions in order to consolidate the findings and discuss the rational behind the conclusions.}
 
 % In this ecosystem, experts who may not be officially part of an SLR, can contribute to the study and alleviate some of the complications by using their expertise. Survey participants emphasized the importance of involving the experts in this process. One participant mentioned: " Librarians offer so many tips. They advised me on selecting the appropriate digital databases. Also, they helped me with designing the search strategies.". A Ph.D. student highlighted the impact of supervisors’ advice in its SLR experience.
% Here we summarize the roles that the survey participants believe the individuals can play to help with SLR process and decrease the workloads for the authors: The survey participants believe that developing more tools are required to help them in conducting SLRs. They highlighted that it is inevitable to using machine learning technologies to help SLR process. Problems such as managing large dataset of citations or managing the references are impossible to be done manually.\\
% Maisie Added this 
% As a result we argue that when the SLR author has more experience and knowledge among the research topic he/she would face less difficulty. This correlation is more evident when the task requires more human intervention and decision making.\\


% \begin{figure}[H]
% \caption{Challenge Factors and the Implications}
% \label{fig:ChallengeFactors}
% \includegraphics[width=8cm]{Image/ChallengeFactors.pdf}
% \end{figure}


% \small{\color{gray}\textit{
% "When the topic under SLR is new for me, it is difficult to create an initial map of the researched topics or to identify relevant terms to compose the search strings;"}}


% Because of this, we use two different tests of independence for each pair of factors. For pairs of one numeric and one categorical, we used Kruskal-Wallis (\textit{kw}), and 



Intro for future 

SLRs are meant to provide a high level of evidence on the effectiveness of interventions in healthcare studies, while in other disciplines (such as software engineering), they usually provide a summary of the current advancements in a research topic to define future research objectives.
The automated tools would be advantageous to the researchers to undertake more SLRs and produce more reliable studies.

Systematic Literature Review (SLR) is a fundamental component in different research disciplines. However, conducting an SLR over requires tremendous effort and presents several challenges. Methodological challenges of SLR studies involving different dimension for which many novice researchers are not well equipped or prepared for. Due to these challenges, some researchers and software developers explored implementing automation techniques to help SLR researchers. 
Despite these endeavors, producing an SLR stays as an expensive and laborious experience for researchers. In this paper, We report on a survey conducted in SLR authors. We aimed to bring to light the real challenges related to the researchers’ experiences and practical concerns. We urged the participants to share the workarounds they exposed to overcome these challenges as well as their concerns for adopting automation techniques in this process. This experience paper makes the accounts of the survey participant research journey heard and beneficial to other novice and/or experienced researchers.\\ 
Our results reveal several key findings that can help to build an active SLR ecosystem. It also provides the empirical foundation for providing recommendations to tools developers on how to develop new SLR tools or improve the existing ones.\\
\textbf{Keywords:} Systematic Literature Review; Challenges; Solutions; Qualitative Analysis
\section{Introduction}
Systematic Literature Review (SLR) is a well-known, comprehensive and transparent research methodology that is popularly adopted in different disciplines. SLRs are mainly conducted to identify the knowledge gap and explore the state-of-the-art of a research topic. The SLR ecosystem's body comprises senior researchers who conduct SLRs to build a theoretical framework to conceptualize the study in a broader context and present the gap in the literature; and the younger researchers (e.g., Ph.D. students) who conduct SLRs to advance their knowledge in a research topic.\\
Despite the advantage of SLRs to the science, conducting an SLR remains a time-consuming and complicated process that is prone to human errors. Conducting an SLR requires a combination of domain knowledge and the information resources that is available to all (e.g., systematic review guidelines) as well as the implicit knowledge that stays in domain expert’ heads (e.g., the knowledge for formulating research questions). Therefore, in addition to the challenges that arise due to the nature of the process (e.g., screening a large number of studies), some challenges are more specific to the authors who conduct SLR. These challenges may affect SLR development practices, velocity, and quality of the studies. However, not much is known about the impact of these challenges and the workarounds that are adopted by the SLR authors to mitigate these challenges.\\ 
The SLR challenges make it a suitable candidate to receive aid from automation techniques~\cite{riaz2010experiences}.  Consequently, Achieving a deeper understanding of how SLR ecosystem works will guide tool designers for developing more efficient tools that suit SLR authors requirements. In this paper,we explore the challenges that SLR authors encounter, as well as the solutions and workarounds they employ to mitigate these challenges. We report on an online survey with SLR authors that contribute to an SLR development in the recent years. We wanted to uncover the demographics of the SLR authors participating in this community, and we aimed to understand what channels and tools these developers use to support their SLR process.\\
Through a qualitative analysis of collected data, our survey revealed the techniques and communication channels that SLR authors find essential to their work, and we uncovered the challenges they face. We believe this information can utilize the design of SLR tools. We also anticipate that this study can be used as guideline for novice reviewers and highlight the real challenges of SLR. These insights have led to several recommendations on how to build an active collaborative ecosystem for conducting SLR. Additionally, Our initial literature review indicates that SLR requires significant amount of manual works and some attempts to automate to use automation techniques such as machine learning and crowdsourcing techniques to reduce this workload. However, studies show that the these techniques are not practically used in the real SLR scenarios~\cite{al2019identification,carver2013identifying}.
In this study, we are systematically gather and analyze information from SLR authors about the challenges they face, as well as workarounds they employ individually to overcome these hurdles. Also, we investigate the exiting concerns that researchers have about the new SLR community. Our work investigates the following research questions:\\
\textbf{RQ1 - } What challenges do SLR authors face when conducting SLR and to what extent they experience these challenges?\\
\textbf{RQ2 - }What solutions do these researchers employ to overcome these challenges and support SLR activities?\\
The remainder of this paper is organized as follow:\\ 
Section~2 provides an overview of the SLR process, and related works;\newline 
Section~3 describes the research methodology(research questions, survey design, survey distribution, data gathering, analysis methods and participants demographics;\newline 
Sections~4 presents study results regarding the SLR challenges;\newline 
Sections~5 presents study results regarding the solutions;\newline Section~6 discusses the implications of the results;\newline 
Section~7 describes the limitations and threats to validity;\newline
Finally, Section~8 concludes the paper.


Because the contextual inquiry gets the researcher much closer to the actual setting, the results may be considered stronger and more transferable in the future.


It is necessary at taking into account the effects of last type of challenges on SLR production, however, not much is known about, neither about the impact of these challenges, nor the solutions that are adopted by to mitigate them.\\

% Additionally, Our initial literature review indicates that SLR requires significant amount of manual works and some attempts to automate to use automation techniques such as machine learning and crowdsourcing techniques to reduce this workload. However, studies show that the these techniques are not practically used in the real SLR scenarios~\cite{al2019identification,carver2013identifying}.


% \begin{table*}[h]
% \caption{The codes used to categorize solutions shared by the participants to overcome these challenges} 
% \label{table:Findings_Solutions}
% \begin{tabular}{p{14cm}}
% \toprule
% \textbf{Solutions Strategy}\\
% \toprule
% \textit{\textbf{Employing external human resources(crowds)}} \\
% \hspace{20pt} • Establishing relationship with external experts to share knowledge and experience when human resource is scared;\\
% \hspace{20pt} • Sharing research resources (e.g., data sharing) through collaboration channels when needed; \\
% \hspace{20pt} • Novice researchers gain experience and credibility by performing small tasks in cooperation with senior researchers;\\
% \hspace{20pt} • Researchers from different geographic areas are given the chance to be part of high profile research;\\
% \hspace{20pt} • Experts from other tribes can help to develop tools and services aid conducting SLRs;\\
% \hspace{20pt} • Implemented tools and methods to overcome challenges can be shared with others;\\
% \arrayrulecolor{black!20}\midrule
% \textit{\textbf{Adopting tools and automation techniques}}\\
% \hspace{20pt} • Some tasks are eligible to be automated at some level machine learning and data mining techniques;\\
% \hspace{20pt} • Automating tasks would help the researcher to focus more on the tasks that require more human-interaction;\\
% \arrayrulecolor{black!20}\midrule
% \textit{\textbf{Learning from the best practice}}\\
% \hspace{20pt} • Following best practices (e.g., published reviews) is another way to find valuable information regarding SLR process.\\
% \arrayrulecolor{black}\bottomrule 
% \end{tabular} 
% \end{table*}


% \begin{table*}[h]
% \caption{This shows how the codes are used to categorize challenges shared by the participants and based on findings that emerged from the analysis. It also shows strategies shared with the participants as solutions to overcome these challenges} 
% \label{table:Findings_Challenges}
% \begin{tabular}{p{13cm}}
% \toprule
% \textbf{Challenges Category}\
% \arrayrulecolor{black!20}\midrule
% \textit{\textbf{Insufficient human resources}} \\
% • Inadequate experience in conducting SLR or knowledge gap about the research topic;\\
% • Lack of knowledge about existing solutions/workarounds that aid SLR process;\\
% \arrayrulecolor{black!20}\midrule
% \textit{\textbf{Collaboration issues}}\\
% • Collaboration with external resources difficulties; \\
% • Insufficient channels for collaboration and sharing knowledge among researchers;\\
% • Intellectual Property(IP) security and ownership breaching when sharing with external resources;\\
% \arrayrulecolor{black!20}\midrule
% \textit{\textbf{Scarce research funding}} \\
% • High cost of human resources prevents researchers for developing new tools or exploring existing tools; \\
% • It is costly to access published literature. In addition, publishing in open access format is also expensive;\\
% • High cost of applications subscription, hurdles using the existing tools;\\
% \arrayrulecolor{black!20}\midrule
% \textit{\textbf{Data accessibility restrictions}}\\
% • Prohibitive access to published literature;\\
% • Restricted access to data for developing SLR automation;\\
% \arrayrulecolor{black}\bottomrule 
% \end{tabular} 
% \end{table*}


\begin{table*}[t]
\small
\caption{Survey Questions}
\label{table:SurveyQuestions}
\vspace{-0.3cm}
\begin{tabular}{p{0.5cm}|p{0.5cm}|p{12cm}}
\toprule
\textbf{\#} & \textbf{RQ}&\textbf{ Survey Question}\\
\toprule
&&\hspace{100pt}\textit{\textbf{General Question}}\\
\arrayrulecolor{black!20}\midrule
Q1 &Dem& Please answer the following questions about your experience in conducting SLR\\
1.1 && How many SLRs have you conducted?\\
1.2 && How many reviewers were involved in conducting these reviews? \\
1.3 && How long did it take to complete these reviews on average? \\
1.4 && What was the research area of these SLRs? \\
1.5 && What was your status when conducting the SLR(s)? (e.g., Ph.D student) \\
\arrayrulecolor{black}\midrule
&&\hspace{100pt}\textit{\textbf{Planning Phase}}\\
\arrayrulecolor{black!20}\midrule
Q2&& Please choose options that express your experience in performing following SLR tasks:\\
 2.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
 2.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
\arrayrulecolor{black!5}\midrule
T2.1&&\hspace{4pt}Finding previous secondary studies (e.g., SLRs)  \\
T2.2&&\hspace{4pt}Defining research questions \\
T2.3&&\hspace{4pt}Defining study search strategy (e.g., what databases to search, defining the search keywords)\\
T2.4&&\hspace{4pt}Defining data collection method (e.g. data extraction template)\\
\arrayrulecolor{black!5}\midrule
Q3&RQ1&Please describe challenges you faced while performing any tasks related to these phase of SLR.\\
Q4&RQ2&Please describe if you developed any solution or work-around to overcome the challenges of conducting these tasks.\\
Q5&RQ2&If you used tools or platforms for conducting these tasks, what did you like or dislike about them? If you didn't use any tool( due to its limitations) what possible solution do you wish available or analogous to tools in other fields?\\
Q6&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
\arrayrulecolor{black}\midrule
&&\hspace{100pt}\textit{\textbf{Conducting Phase}}\\
\arrayrulecolor{black!20}\midrule
Q7&&Please choose options that express your experience in performing following SLR tasks:\\
 7.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
 7.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
\arrayrulecolor{black!5}\midrule
T7.1&&\hspace{4pt}Building the search queries for each database\\
T7.2&&\hspace{4pt}Retrieving and storing retrieved studies\\
T7.3&&\hspace{4pt}Applying inclusion and exclusion criteria to filter studies\\
T7.4&&\hspace{4pt}Screening titles and abstracts\\
T7.5&&\hspace{4pt}Assessing the quality of the remaining studies \\
T7.6&&\hspace{4pt}Extracting data from selected studies \\
T7.7&&\hspace{4pt}Annotating and tagging for specific data categories (e.g.,PICO)\\
\arrayrulecolor{black!5}\midrule
Q8&RQ1&Please describe challenges you faced while performing these tasks related.\\
Q9&RQ2&Please describe any solution or work-around you developed to overcome these challenges\\
Q10&RQ2&If you used tools or platforms for conducting these tasks, what did you like or dislike about them?If you didn't use any tool( due to its limitations) what possible solution do you wish available or analogous to tools in other fields?\\
Q11&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
\end{tabular}
\end{table*}
\begin{table*}  %second part
\begin{tabular}{p{0.5cm}|p{0.5cm}|p{12cm}}
\title{}
&&\hspace{100pt}\textit{\textbf{Reporting Phase}}\\
\arrayrulecolor{black!20}\midrule
Q12&& Please choose options that express your experience in performing following SLR tasks:\\
 12.1&RQ1&\hspace{2pt} The task is time-consuming/complex (Agree/Disagree) \\
 12.2&RQ2&\hspace{2pt} Did you use any tools to perform this task? (please name the tools)\\
\arrayrulecolor{black!5}\midrule
T12.1&&\hspace{4pt}Documenting the findings\\
T12.2&&\hspace{4pt}Analyzing and synthesizing collected data\\
T12.3&&\hspace{4pt}Writing the report\\
\arrayrulecolor{black!5}\midrule
Q13&RQ1&Please describe challenges you faced while performing any tasks related to this phase.\\
Q14&RQ2&Please describe any solution or work-around that you developed or aware of, to overcome these challenges.\\
Q15&RQ1&What barriers do you see in employing automation techniques (e.g., machine learning, crowdsourcing) in performing these tasks?\\
\arrayrulecolor{black}\bottomrule 
\end{tabular}
\end{table*}



%They also seem very keen to try alternative solutions and workarounds to overcome these difficulties. 


\item Despite the DLs limitation that results in this noise, some participants mentioned that topic and scope of the study could also affect the level of these difficulties.~ P25 mentioned~\textit{" This task is very time-consuming. I wish there was a tool that was getting the keywords and screen the papers to find similar ones, and return some similarity rating. This would help a lot, rather than screening 100s of papers!"}. 


% \subsection{Studies on the challenges and pitfalls in the SLR process}
% In a related work, Al-Zubidy et al.~\cite{al2019identification} investigated the challenges associated with the SLR search process. In their study, they conducted an SLR and surveyed SLR authors of the software engineering (SE) community. They compared the result of their SLR to the outcome of the survey to find the correlation between the problems identified by the literature to the real issues among the SLR authors.The authors also reported the desired tools requirements for the SLR search phase as a result of their survey. They showed that SLR search process in the SE domain still experiences a large number of barriers, and there is still the need for additional work towards automating this process.

% Carver et al.~\cite{carver2013identifying} conducted a survey study to identify the most challenging and time-consuming tasks in SLR process. Their survey result indicated that the search phase as one of the most time-consuming task that requires more tool support. 

% Through an experimental study, Riaz et al.~\cite{riaz2010experiences} reported the comparison result of experiences from three PhD students with carrying out SLRs to the experience of the senior researchers when undertaking an SLR. They aimed to understand if the challenges faced by novices in terms of time taken to conduct the review is different from those faced by expert researchers. They reported that while some problems are faced by both novices and experts, many others are specific to novices, where the help of domain and SR experts can solve some of these issues.

% Furthermore, previous research investigated on challenges of conducting SLR in diverse demographics of the research community. 

% Sandy Oliver et al.~\cite{oliver2015capacity} explored these challenges in the healthcare domain within low and middle-income countries (LMICs). They explored the current capacity and the activities that could improve SLR production in these countries. The result of their study showed that the limited capacity for conducting systematic reviews within LMICs presents a major challenge to improving their health systems. They also presented that effective capacity in these countries can be developed through funding at multiple levels simultaneously, supported by high-income countries with established facilities and expertise.

% \subsection{Collaboration and automation in the SLR process}
% Extensive work has been done by the Software Engineering research community in the context of automating SLR tasks in order to alleviate SLR-related challenges. There are two main research streams in this context. The first group of researchers who explored and proposed machine learning and data mining techniques to (semi-automate) SLR tasks ~\cite{lanera2018extending,marcos2018decision,goswami2019effective,olorisade2019use,alamri2015automatic,cohen2015automated,gotz2018supporting,Almeida2016,Adeva2014,Fabbri2016,kontonatsios2017,langlois2018}, and the second group who are exploring the advantage of employing the crowds to help within this process~\cite{brown2014using,Wallace2017,krivosheev2018}.

%Despite many studies showing the common challenges of conducting SLR, none of these studies focused on the rationals behind these challenges. Yet, in this study, we aim at increasing our empirical knowledge on this field by a quantitative research. We gather and analyze the real challenges and reasons behind them. We also explore the solutions that the members of the research community employ to overcome these challenges.

==> Image/Backup/test.tex <==
In this section we describe our ongoing exploration into the technical feasibility of our approach.\\
We started with \textit{article recommendation} as it emerged as a promising component based on the feedback from SLR authors, but raised concerns in terms of feasibility. We note however that providing support for identifying related SLRs has all  the potential benefits but fewer of the concerns (e.g., recall and accuracy) with respect to assisting the identification and screening of relevant literature~\cite{kontonatsios2017semi}. In the planning, bringing up the most relevant SLRs and papers can provide the additional context in a task that some people are not even aware of. 


\indent\textbf{Prototype}. The prototype is our initial exercise into understanding the technical requirements of the system, as well as a working tool to serve evaluation purposes. On the surface, the current version of the prototype provides a set of REST APIs (and an accompanying user interface) that given a set of RQs in input, it returns the most relevant SLRs, along with the relevance score computed based on the available models. 
Fig.~\ref{fig:Pipeline} presents the pipeline of the implementation.

The source of information is currently a curated database of SLRs, where domain-specific information has been manually extracted so as to evaluate the recommendation component in isolation. The end goal is to have a data layer that can interface with existing services to access structured and unstructured data, which can then be processed to automatically extract relevant domain-specific information. 
While we currently use a MySQL database to store and retrieve raw and curated data, the concept of \textit{Data Lake} \cite{beheshti2017coredb} emerges as a promising direction to store and query structured and unstructured SLR data. 

\begin{figure*} 
\centering
\includegraphics[width=\textwidth]{Image/Pipeline_Final.pdf}
\caption{Architecture Pipeline} \label{fig:Pipeline}
\end{figure*}

In entering the augmentation layer, the data is pre-processed in two steps: (a) normalizing text corpus (e.g., removing special characters and stop words, all to lowercase); and (b) lemmatizing and converting each word to its base form. We leverage Stanford CoreNLP toolkit\footnote{https://nlp.stanford.edu/software/tagger.html} to perform this process.

Following the data cleaning, the next step is to extract meaningful information from the data.
The inspiration behind our proposed approach is leveraging a similar approach to the word embedding's model~\cite{mikolov2013distributed} that represents words in a Vector Space Model (VSM). We have extended the idea of considering a "word" as a vector to represent the SLR-related corpus (e.g., RQs and SLR abstracts) in a vector space. To create the VSMs, we employ an N-gram selector component to extract all the keywords (nouns and verbs) from sentences of the given context. We leverage Stanford Part-Of-Speech (POS) Tagger~\cite{manning2014stanford} to achieve this. 

Then, we create a list of n-grams out of these keywords and transform them into vector representations for each corpus. After encoding the given corpora into vectors, these vectors are used to calculate the similarity between desired corpora.

Information is then augmented based on a pool of word embedding models. Our work leverages state-of-the-art algorithms widely used in NLP communities. Several such algorithms (e.g. GloVe~\cite{pennington2014glove}, Word2Vec~\cite{mikolov2013efficient}, Numberbatch~\cite{speer2016conceptnet}, WikiNewsFast~\cite{bojanowski2017enriching}, and GoogleNews~\cite{church2017word2vec}) come with efficient implementations that are readily available as libraries to use.

The REST APIs then expose the functionality of the article recommendation component for programmatic access. A front-end application takes these services and wraps them up in a user interface.

\smallskip
\indent\textbf{Planned Evaluation}.
The goal of the initial evaluation is to inform specific design decisions regarding the algorithmic support for recommending papers. Among the main design decisions we consider: i) \textit{What models will better serve the specific task?}
 The idea is to identify among the embedding models and architectures the most promising candidates to build on, and understand whether investing in domain-specific embedding models is required. Then, ii) \textit{What information should we leverage when assessing the relevance calculations?} (e.g., title, title-abstract, RQs, full-text). The aim is to understand what (combinations of) information to focus when assessing the relevance of SLRs from an input RQs, and therefore to consider in the extraction process. 

The prototype supports these two dimensions, models and selective information, so as to serve the evaluations. The dataset of SLRs is being manually constructed to incorporate for each SLR a set of related SLRs (as reported in the reviews) and not relevant SLRs as judged by human experts. 

Armed with the human-annotated dataset, we evaluate the quality of word embedding models by assessing how well the similarity scores of the word vectors correlate with human judgment~\cite{shi2017jointly}. The similarity is calculated as the distance between the vectors representing RQs and SLRs, using cosine similarity as measure, which has been found suitable for SLRs in prior work \cite{lopes2007visual}.

We rely on Spearman’s rank $(r_s)$ correlation between the word embedding models similarity score and researchers annotations to evaluate how well the similarity of the given pairs (e.g., RQs and abstracts) agrees with human judgments~\cite{huang2012improving}.
We performed a preliminary test run to tune the experimental setup, and the early results are encouraging. Results under limited settings (e.g., dataset of 160 SLRs, only abstract-RQ comparisons) already show good level of agreement (rs = 0.67), for the best performing model, although at this point this is anecdotal since more comprehensive tests are required.  
